AdaShadow: Responsive Test-time Model Adaptation in Non-stationary Mobile Environments

On-device adapting to continual, unpredictable domain shifts is essential for mobile applications like autonomous driving and augmented reality to deliver seamless user experiences in evolving environments. Test-time adaptation (TTA) emerges as a promising solution by tuning model parameters with unlabeled live data immediately before prediction. However, TTA's unique forward-backward-reforward pipeline notably increases the latency over standard inference, undermining the responsiveness in time-sensitive mobile applications. This paper presents AdaShadow, a responsive test-time adaptation framework for non-stationary mobile data distribution and resource dynamics via selective updates of adaptation-critical layers. Although the tactic is recognized in generic on-device training, TTA's unsupervised and online context presents unique challenges in estimating layer importance and latency, as well as scheduling the optimal layer update plan. AdaShadow addresses these challenges with a backpropagation-free assessor to rapidly identify critical layers, a unit-based runtime predictor to account for resource dynamics in latency estimation, and an online scheduler for prompt layer update planning. Also, AdaShadow incorporates a memory I/O-aware computation reuse scheme to further reduce latency in the reforward pass. Results show that AdaShadow achieves the best accuracy-latency balance under continual shifts. At low memory and energy costs, Adashadow provides a 2x to 3.5x speedup (ms-level) over state-of-the-art TTA methods with comparable accuracy and a 14.8% to 25.4% accuracy boost over efficient supervised methods with similar latency.

==> body/imple_and_eval.tex <==

\subsection{Experiment Setup}
\noindent \textbf{Models.} We evaluate TETTA using three widely employed NN models: VGG16 (without BN layer)\cite{}, MobileNetV2 (with BN layer)\cite{}, and ResNet-50 (with BN layer)\cite{}. These models are chosen for their diverse architectures and computation complexities.

\noindent \textbf{Datasets.} Following the previous TTA methods\cite{}, we evaluate models with {CIFAR10, CIFAR10C},{CIFAR100, CIFAR100C} where the first and the second dataset in each group refers to the cloud and the mobile dataset.      
CIFAR10C and CIFAR100C include 15 types of distribution shift generated by different artificial corruptions, such as Gaussian noise. However, artificial corruptions can't completely simulate the real distribution shifts caused by natural factors, such as lighting conditions, shadows, shooting angles, and so on.
To validate model performance in real mobile scenarios, we further conduct evaluations on NICO++\cite{}. NICO++ is a dataset collected from various natural environments, including autumn, dim, grass, outdoor, rock, and water scenes.

For {CIFAR10, CIFAR10C}, model is initially pre-trained on CIFAR10. Subsequently, we conduct continuous tests on 15 corruptions without resetting model, which is more challenging than previous offline adaptation on single scene but more realistic. A similar setup is employed for {CIFAR100, CIFAR100C}.
For NICO++, model is initially pre-trained on outdoor scene data and then we conduct continuous tests different scenes in the order of autumn->dim->grass->rock->water->autumn->dim->grass->rock->water.

\noindent \textbf{Evaluation Metric.}
For all experiments, we report both inference results accuracy and adaptation efficiency. To represent intuitive acceleration on data stream inference of the methods, we use inference throughput——frame per second (fps), instead of latency metrics to indicate the efficiency of model inference.

\noindent \textbf{Hardware setup.}
We evaluate all methods on embedded devices including Nvidia Jetson NX, Nvidia Jetson Nano and Raspberry Pi 4B. These AI computing devices are widely used in mobile embedded platforms such as drones\cite{} and robots\cite{}. Jetson NX is equipped with an Nvidia Pascal GPU with 256 CUDA cores, Cortex-A57 CPU, and 8GB shared memory between GPU and CPU.
Jetson Nano is equipped with an Nvidia Maxwell GPU with 128 CUDA cores, Cortex-A57 CPU, and 4GB shared memory between GPU and CPU. 
Raspberry Pi 4B is equipped with a 1.5GHz Cortex-A72 CPU and 4GB memory.
On Jetson NX, we installed the Jetpack 4.6.4 OS based on Ubuntu 18.04. On Raspberry Pi, we installed the 64-bit Raspbian 11 OS.

\noindent \textbf{Comparison Baselines.}
In continuous scenes, basic baselines include update all parameters (AllUpdate). To compare accuracy and efficiency of our method, We primarily selected TTA and sparse update methods.
\textbf{TTA methods} includes classical methods TENT\cite{wang2021tent} and SOTA methods EATA\cite{niu2022efficient}, CoTTA\cite{wang2022continual}, and memory-efficient method EcoTTA\cite{song2023ecotta}.
\textbf{Sparse update methods} includes Tiny Training Engine(TTE)\cite{lin2022device}, and ElasticTrainer\cite{huang2023elastictrainer}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Overall Performance}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Adaptation with Natural Shift Data}
\label{Adaptation with Natural Shift Data}
%我们首先在NICO++数据集上将我们的方法Chameleon与其他基线方案进行对比，以模拟具有不同自然环境（季节、背景、光线）的连续移动场景。我们使用Nvidia Jetson NX设备和ResNet50模型进行测试，测试批次大小是4，并将speedup objective $\sigma$设置为0.33以实现三倍适应加速的目标。我们按时间顺序不断切换场景（例如autumn、dim）并用新场景数据更新模型，场景切换循环执行两个round。我们报告模型适应后的推理精度，和执行在线适应与推理后的数据吞吐量。
%表\ref{table_1}的结果表明，与完整更新模型相比，Chameleon通过稀疏的backward和reforward实现了三倍左右的推理加速。并且AllUpdate方法由于在每次适应中更新所有参数，在连续label-free的条件下受unreliable伪标签的影响，精度不断降低到5.4%。和TTA方法相比，Chameleon在保持相似精度的情况下，普遍实现了2x~3x的加速，相比CoTTA甚至加速了18.2x。Chameleon相比于TENT、EATA还具有更高的精度，因为这些方法只更新BN层，限制了模型的优化空间。而CoTTA和EcoTTA由于更新更多参数导致更长的适应时延，从而降低了推理吞吐量。和sparse update方法相比，Chameleon同时提升了推理吞吐量和精度指标。Chameleon对每一批输入数据都实时评估和更新层精度重要性，因此相比于TTE离线评估和ElasticTrainer定期评估，Chameleon具有更高的适应精度。TTE针对峰值内存优化而设计的稀疏更新方案并没有为时延带来优化。ElasticTrainer实现了2x左右的加速，但由于缺少准确的在线层时延和缺少对reforward的优化，吞吐量依然比Chameleon低约19fps。此外，可以发现几乎所有方法都在2nd round中达到了比1st round更高的精度。因为相比适应单个场景后重置模型，持续适应能够保持模型对历史场景的记忆并在遇到相似场景时基于已有历史知识更快适应。



% Table 1
\begin{table*}[]
\centering
\scriptsize
\caption{Table 1.}
\renewcommand{\arraystretch}{1.2}
\scalebox{1.2}{
\begin{tabular}{|c|cccccccccc|c|c|}
\hline
\textbf{Time}   & \multicolumn{10}{c|}{\textbf{t   ———————————————————————————————————————————————————————\textgreater{}}}                                                                                                                                                                                                                                                                  & \multirow{3}{*}{\textbf{Mean ACC.(\%)}} & \multirow{3}{*}{\textbf{Th.(fps)}} \\ \cline{1-11}
\textbf{Round}  & \multicolumn{5}{c|}{\textbf{1}}                                                                                                                                                           & \multicolumn{5}{c|}{\textbf{2}}                                                                                                                                      &                                     &                                           \\ \cline{1-11}
\textbf{Method} & \multicolumn{1}{c|}{\textbf{Autumn}} & \multicolumn{1}{c|}{\textbf{Dim}} & \multicolumn{1}{c|}{\textbf{Grass}} & \multicolumn{1}{c|}{\textbf{Rock}} & \multicolumn{1}{c|}{\textbf{Water}} & \multicolumn{1}{c|}{\textbf{Autumn}} & \multicolumn{1}{c|}{\textbf{Dim}} & \multicolumn{1}{c|}{\textbf{Grass}} & \multicolumn{1}{c|}{\textbf{Rock}} & \textbf{Water} &                                     &                                           \\ \hline
AllUpdate       & \multicolumn{1}{c|}{72.0}            & \multicolumn{1}{c|}{51.4}         & \multicolumn{1}{c|}{47.0}           & \multicolumn{1}{c|}{40.3}          & \multicolumn{1}{c|}{26.1}           & \multicolumn{1}{c|}{23.4}            & \multicolumn{1}{c|}{13.9}         & \multicolumn{1}{c|}{9.4}            & \multicolumn{1}{c|}{9.1}           & 5.4            & 29.8                                & 24.0                                      \\ \hline
TENT            & \multicolumn{1}{c|}{84.2}            & \multicolumn{1}{c|}{81.8}         & \multicolumn{1}{c|}{86.6}           & \multicolumn{1}{c|}{86.2}          & \multicolumn{1}{c|}{86.5}           & \multicolumn{1}{c|}{89.9}            & \multicolumn{1}{c|}{89.1}         & \multicolumn{1}{c|}{91.3}           & \multicolumn{1}{c|}{90.9}          & 91.7           & 87.8                                & 30.1                                      \\ \hline
EATA            & \multicolumn{1}{c|}{85.2}            & \multicolumn{1}{c|}{83.0}         & \multicolumn{1}{c|}{87.5}           & \multicolumn{1}{c|}{86.6}          & \multicolumn{1}{c|}{86.1}           & \multicolumn{1}{c|}{90.1}            & \multicolumn{1}{c|}{89.8}         & \multicolumn{1}{c|}{92.2}           & \multicolumn{1}{c|}{91.8}          & 91.7           & 88.4                                & 27.4                                      \\ \hline
CoTTA           & \multicolumn{1}{c|}{85.0}            & \multicolumn{1}{c|}{83.3}         & \multicolumn{1}{c|}{87.7}           & \multicolumn{1}{c|}{86.3}          & \multicolumn{1}{c|}{85.8}           & \multicolumn{1}{c|}{90.3}            & \multicolumn{1}{c|}{89.2}         & \multicolumn{1}{c|}{92.4}           & \multicolumn{1}{c|}{90.5}          & 91.2           & 88.2                                & 4.2                                       \\ \hline
EcoTTA          & \multicolumn{1}{c|}{85.4}            & \multicolumn{1}{c|}{84.9}         & \multicolumn{1}{c|}{88.3}           & \multicolumn{1}{c|}{87.4}          & \multicolumn{1}{c|}{86.5}           & \multicolumn{1}{c|}{91.7}            & \multicolumn{1}{c|}{90.7}         & \multicolumn{1}{c|}{92.9}           & \multicolumn{1}{c|}{91.9}          & 92.3           & 89.2                                & 23.8                                      \\ \hline
TTE             & \multicolumn{1}{c|}{74.7}            & \multicolumn{1}{c|}{71.8}         & \multicolumn{1}{c|}{77.5}           & \multicolumn{1}{c|}{76.0}          & \multicolumn{1}{c|}{74.9}           & \multicolumn{1}{c|}{79.8}            & \multicolumn{1}{c|}{78.2}         & \multicolumn{1}{c|}{80.7}           & \multicolumn{1}{c|}{80.0}          & 81.5           & 77.5                                & 29.5                                      \\ \hline
ElasticTrainer  & \multicolumn{1}{c|}{78.5}            & \multicolumn{1}{c|}{76.1}         & \multicolumn{1}{c|}{79.9}           & \multicolumn{1}{c|}{80.4}          & \multicolumn{1}{c|}{78.5}           & \multicolumn{1}{c|}{82.5}            & \multicolumn{1}{c|}{83.2}         & \multicolumn{1}{c|}{84.5}           & \multicolumn{1}{c|}{84.7}          & 84.7           & 81.3                                & 57.6                                      \\ \hline
Ours            & \multicolumn{1}{c|}{86.9}            & \multicolumn{1}{c|}{84.8}         & \multicolumn{1}{c|}{89.0}           & \multicolumn{1}{c|}{88.5}          & \multicolumn{1}{c|}{87.7}           & \multicolumn{1}{c|}{91.6}            & \multicolumn{1}{c|}{91.0}         & \multicolumn{1}{c|}{93.7}           & \multicolumn{1}{c|}{92.9}          & 92.9           & \textbf{89.9}                       & 76.4                                      \\ \hline
\end{tabular}
}
\label{exp:table_1}
\end{table*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent \textbf{Adaptation with Corruption Data.}
%我们在CIFAR10C/100C上展开round=1的测试，以模拟具有不同图像干扰（模糊、噪声、遮挡物）的连续移动场景，并保持和\ref{Nvidia Jetson NX设备和ResNet50}相同的hardware、model and speedup objective。我们分别选择了两个最具有代表性的TTA方法EATA和sparse update方法ElasticTrainer报告结果。
%表\ref{table_2}的结果表明，Chameleon有效地提升了推理速度（fps）和精度。相比于EATA，Chameleon实现了3x左右的加速而不损失推理精度。ElasticTrainer尽管能有限提高推理吞吐量，但由于定期层重要性评估无法捕获到实时数据变化带来的层重要性变化，准确率比Chameleon低8\%左右。






% Table 2
\begin{table*}[]
\centering
\scriptsize
\caption{Table 2.}
\renewcommand{\arraystretch}{1.2}
\scalebox{1}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|cc|ccccccccccccccc|c|c|}
\hline
\multicolumn{2}{|c|}{Time}                                        & \multicolumn{15}{c|}{t   ——————————————————————————————————————————————————————————————————\textgreater{}}                                                                                                                                                                                                                                                                                                             & \multirow{2}{*}{Mean ACC.(\%)} & \multirow{2}{*}{Th.(fps)} \\ \cline{1-17}
\multicolumn{1}{|c|}{Dataset}                    & Method         & \multicolumn{1}{c|}{Gaus.} & \multicolumn{1}{c|}{Shot} & \multicolumn{1}{c|}{Impu.} & \multicolumn{1}{c|}{Defo.} & \multicolumn{1}{c|}{Glas.} & \multicolumn{1}{c|}{Moti.} & \multicolumn{1}{c|}{Zoom} & \multicolumn{1}{c|}{Snow} & \multicolumn{1}{c|}{Fros.} & \multicolumn{1}{c|}{Fog}  & \multicolumn{1}{c|}{Brig.} & \multicolumn{1}{c|}{Cont.} & \multicolumn{1}{c|}{Elas.} & \multicolumn{1}{c|}{Pixe.} & Jpeg &                                &                           \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{CIAFR10C}}  & EATA           & \multicolumn{1}{c|}{69.4}  & \multicolumn{1}{c|}{71.5} & \multicolumn{1}{c|}{71.6}  & \multicolumn{1}{c|}{83.5}  & \multicolumn{1}{c|}{70.6}  & \multicolumn{1}{c|}{81.8}  & \multicolumn{1}{c|}{85.9} & \multicolumn{1}{c|}{79.5} & \multicolumn{1}{c|}{83.1}  & \multicolumn{1}{c|}{86.1} & \multicolumn{1}{c|}{87.1}  & \multicolumn{1}{c|}{86.8}  & \multicolumn{1}{c|}{75.1}  & \multicolumn{1}{c|}{83.1}  & 73.1 & 79.2                           & 27.5                      \\ \cline{2-19} 
\multicolumn{1}{|c|}{}                           & ElasticTrainer & \multicolumn{1}{c|}{58.6}  & \multicolumn{1}{c|}{64.9} & \multicolumn{1}{c|}{64.8}  & \multicolumn{1}{c|}{77.8}  & \multicolumn{1}{c|}{62.9}  & \multicolumn{1}{c|}{75.4}  & \multicolumn{1}{c|}{79.3} & \multicolumn{1}{c|}{73.7} & \multicolumn{1}{c|}{76.5}  & \multicolumn{1}{c|}{74.2} & \multicolumn{1}{c|}{78.7}  & \multicolumn{1}{c|}{80.8}  & \multicolumn{1}{c|}{66.4}  & \multicolumn{1}{c|}{72.2}  & 65.5 & 71.4                           & 58.6                      \\ \cline{2-19} 
\multicolumn{1}{|c|}{}                           & Ours           & \multicolumn{1}{c|}{67.0}  & \multicolumn{1}{c|}{75.4} & \multicolumn{1}{c|}{70.6}  & \multicolumn{1}{c|}{80.6}  & \multicolumn{1}{c|}{71.7}  & \multicolumn{1}{c|}{79.6}  & \multicolumn{1}{c|}{84.7} & \multicolumn{1}{c|}{85.2} & \multicolumn{1}{c|}{85.4}  & \multicolumn{1}{c|}{85.8} & \multicolumn{1}{c|}{89.6}  & \multicolumn{1}{c|}{84.8}  & \multicolumn{1}{c|}{76.6}  & \multicolumn{1}{c|}{82.9}  & 74.8 & 79.6                           & 79.1                      \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{CIAFR100C}} & EATA           & \multicolumn{1}{c|}{49.4}  & \multicolumn{1}{c|}{52.9} & \multicolumn{1}{c|}{51.5}  & \multicolumn{1}{c|}{63.7}  & \multicolumn{1}{c|}{51.2}  & \multicolumn{1}{c|}{60.8}  & \multicolumn{1}{c|}{66.0} & \multicolumn{1}{c|}{66.7} & \multicolumn{1}{c|}{65.8}  & \multicolumn{1}{c|}{68.6} & \multicolumn{1}{c|}{68.9}  & \multicolumn{1}{c|}{69.0}  & \multicolumn{1}{c|}{57.9}  & \multicolumn{1}{c|}{65.1}  & 54.4 & 60.8                           & 24.3                      \\ \cline{2-19} 
\multicolumn{1}{|c|}{}                           & ElasticTrainer & \multicolumn{1}{c|}{42.4}  & \multicolumn{1}{c|}{49.2} & \multicolumn{1}{c|}{44.9}  & \multicolumn{1}{c|}{58.1}  & \multicolumn{1}{c|}{43.3}  & \multicolumn{1}{c|}{55}    & \multicolumn{1}{c|}{61.9} & \multicolumn{1}{c|}{57.1} & \multicolumn{1}{c|}{59.8}  & \multicolumn{1}{c|}{57.6} & \multicolumn{1}{c|}{60.9}  & \multicolumn{1}{c|}{62.9}  & \multicolumn{1}{c|}{50.1}  & \multicolumn{1}{c|}{58.6}  & 49.7 & 54.1                           & 56.9                      \\ \cline{2-19} 
\multicolumn{1}{|c|}{}                           & Ours           & \multicolumn{1}{c|}{50.1}  & \multicolumn{1}{c|}{54.1} & \multicolumn{1}{c|}{49.8}  & \multicolumn{1}{c|}{63.8}  & \multicolumn{1}{c|}{52.6}  & \multicolumn{1}{c|}{63.1}  & \multicolumn{1}{c|}{65.1} & \multicolumn{1}{c|}{66.0} & \multicolumn{1}{c|}{66.5}  & \multicolumn{1}{c|}{65.8} & \multicolumn{1}{c|}{70.8}  & \multicolumn{1}{c|}{69.5}  & \multicolumn{1}{c|}{62.6}  & \multicolumn{1}{c|}{64.5}  & 54.2 & 61.2                           & 76.2                      \\ \hline
\end{tabular}
}
\label{exp:table_2}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Performance with Different Conditions}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\textbf{Speedup objectives}
%稀疏更新能够通过控制加速目标$\sigma \in \left[ 0,1 \right]$来灵活调整时延和推理时延，从而按照用户需求优先优化推理吞吐量或精度。更小的加速目标通过更少的参数更新来降低适应时延以提高推理吞吐量，但这也同时限制了模型的学习能力而导致精度降低。
%图\ref{fig:speed_up_objective}的结果表明，当$\sigma$是0.5或0.8时，Chameleon能够在不损失精度的情况下实现1.1x~2.3x的推理加速。说明在新场景下对模型进行适应时不需要更新所有的参数，优先更新重要的参数能够在保持性能的情况下降低适应时延。而当$\sigma$是0.2时，Chameleon相比基线方法实现了4.8x左右的加速。但开始出现明显的精度损失，说明更新过少的参数开始限制模型在新场景下的学习能力。Source方法尽管达到了138.2fps的推理速度，但也出现了25\%左右的精度损失。因此在实际部署时，可以通过修改$\sigma$在执行任务时动态调整适应时延，以满足用户或任务对推理吞吐量的动态需求。


Fig. \ref{}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.37\textwidth]{figure/speed_up_objective.pdf}
  \caption{Figure for speed up\_objective.}
  \label{fig:speed_up_objective}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent \textbf{Model Architectures}

%不同结构的NN模型在只更新一部分层后的性能效果可能不同。我们使用VGG16,MobileNetV2和ResNet50三种模型，将Chameleon与其他基线方案在进行对比，并设置加速目标$\sigma$为0.5.
%图\ref{fig:Model_Architectures}的结果表明对于，Chameleon能够在不同结构的神经网络上相比现有方法实现2x-3x的加速效果并保持较高推理精度。由于不具有BN结构，只更新BN层的EATA方法无法应用在VGG16模型上。我们发现所有适应方法在ResNet上都取得了比MobileNetV2更高的精度。这可能是因为MobileNetV2的收敛速度较慢\cite{huang2023elastictrainer}而导致单次在线适应无法充分优化模型的参数，而导致精度提升有限。


Fig. \ref{}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.45\textwidth]{figure/Table4-5.pdf}
  \caption{Figure for table4-5.}
  \label{fig:Model_Architectures}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent \textbf{Hardwares}

%不同结构的NN模型在只更新一部分层后的性能效果可能不同。我们使用VGG16,MobileNetV2和ResNet50三种模型，将Chameleon与其他基线方案在进行对比，并设置加速目标$\sigma$为0.5.
%图\ref{fig:Model_Architectures}的结果表明Chameleon能够在不同结构的神经网络上相比现有方法实现2x-3x的加速效果并保持较高推理精度。由于不具有BN结构，只更新BN层的EATA方法无法应用在VGG16模型上。我们发现所有适应方法在ResNet上都取得了比MobileNetV2更高的精度。这可能是因为MobileNetV2的收敛速度较慢\cite{huang2023elastictrainer}而导致单次在线适应无法充分优化模型的参数，而导致精度提升有限。

% Table 3
\begin{table}[]
\centering
\scriptsize
\caption{Table 3.}
\renewcommand{\arraystretch}{1.3}
\scalebox{1.2}{
\begin{tabular}{|c|ccc|ccc|}
\hline
               & \multicolumn{3}{c|}{NICO++}                                     & \multicolumn{3}{c|}{CIFAR10C}                                   \\ \hline
               & \multicolumn{1}{c|}{R-Pi} & \multicolumn{1}{c|}{J-Nano} & J-NX  & \multicolumn{1}{c|}{R-Pi} & \multicolumn{1}{c|}{J-Nano} & J-NX  \\ \hline
EATA           & \multicolumn{1}{c|}{0.51} & \multicolumn{1}{c|}{3.14}   & 25.30 & \multicolumn{1}{c|}{0.43} & \multicolumn{1}{c|}{2.90}   & 27.50 \\ \hline
EcoTTA         & \multicolumn{1}{c|}{0.45} & \multicolumn{1}{c|}{3.10}   & 22.70 & \multicolumn{1}{c|}{0.33} & \multicolumn{1}{c|}{2.50}   & 23.20 \\ \hline
ElasticTrainer & \multicolumn{1}{c|}{1.20} & \multicolumn{1}{c|}{6.90}   & 60.90 & \multicolumn{1}{c|}{1.00} & \multicolumn{1}{c|}{7.30}   & 61.80 \\ \hline
Ours           & \multicolumn{1}{c|}{1.30} & \multicolumn{1}{c|}{8.80}   & 77.36 & \multicolumn{1}{c|}{1.10} & \multicolumn{1}{c|}{8.20}   & 80.20 \\ \hline
\end{tabular}
}
\label{exp:table_3}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Performance in Real-world settings}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Dynamic batch size}

%在真实场景下，推理数据的batch size可能会动态变化，这取决于上一个周期内到达设备并需要推理的样本数量。我们在batch size分别为1、2、4和16的情况下测试了Chameleon的精度、吞吐量和内存指标。表\ref{fig:table_4}的结果表明随着batch size的增加，模型的适应精度从76.5%上升到86.7%。这可能是由于ResNet50中的BN结构导致的，更大的batch有利于统计更准确的信息。吞吐量也从19.2上升至340.2，这是由于GPU针对并行化高度优化的计算结构所导致的。因此，在内存预算充足的情况下，更大的batch size有助于实现更准确和更快的模型适应。

% Table 4
\begin{table}[]
\centering
\scriptsize
\caption{Table 4.}
\renewcommand{\arraystretch}{1.3}
\scalebox{1.5}{
\begin{tabular}{|c|c|c|c|c|}
\hline
                & BS=1 & BS=2 & BS=4 & BS=16 \\ \hline
Accuracy(\%)    & 76.5 & 81.5 & 85.5 & 86.7  \\ \hline
Throughput(fps) & 19.2 & 43.2 & 79.6 & 340.2 \\ \hline
Peak Memory(MB) & 2108 & 2210 & 2462 & 3794  \\ \hline
\end{tabular}
}
\label{exp:table_4}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent \textbf{Dynamic hardware condition}

%TODO:在真实场景下硬件设备的资源信息可能动态变化，这取决于当前设备上并行的其他占用计算和内存资源的进程以及实时设备硬件信息。

Fig. \ref{}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.37\textwidth]{figure/Table9.pdf}
  \caption{Figure for table9.}
  \label{fig:Dynamic_hardware_condition}
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Continuous Data Stream Scene}

%为了测试不同方法在连续数据流输入下（例如无人机探测、自动驾驶、生产线产品检测等）的实时性和准确性，我们模拟了真实环境下的数据输入条件：每一批次数据定时到达，而不管上一批数据是否已经完成推理。我们测试了两种常见应对连续到达数据的推理模式: Inference Immediately and Inference After Adaptation.

\begin{figure}[t]
	\centering 
	\subfloat[]{\label{fig:InferenceImmediately}
		\includegraphics[width=0.92\linewidth]{figure/InferenceImmediately.pdf}}
		\\
	\subfloat[]{\label{fig:InferenceAfterAdaptation}
		\includegraphics[width=0.92\linewidth]{figure/InferenceAfterAdaptation.pdf}}
	\caption{}
	\label{fig:ContinuousInference}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Inference Immediately}

%TODO:第一种模式如图xx所示，当新数据在时刻t到达时，直接选择已经完成适应的最近时刻的模型进行推理，而不需要等待模型基于新数据完成适应后推理。这种推理模式具有最高的实时性，但用历史场景的模型推理当前数据可能会产生精度问题。图\ref{fig:Inference_Immediately}的结果表明

Fig. \ref{}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.45\textwidth]{figure/InferenceImmediately.pdf}
  \caption{Figure for table9.}
  \label{fig:Inference_Immediately}
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent \textbf{Inference After Adaptation}

%TODO:第二种模式如图xx所示，当新数据在时刻t到达时，需要等待模型基于新数据完成适应后再推理新数据。这种推理模式具有最高的准确性，但较高的适应时延会影响推理吞吐量，甚至造成推理数据的等待和堆积问题。如图xx中的红色时间所示，。表\ref{fig:Inference_Immediately}的结果表明

% Table 5
\begin{table}[]
\centering
\scriptsize
\caption{Table 5.}
\renewcommand{\arraystretch}{1.3}
\scalebox{1.25}{
\begin{tabular}{|c|c|c|c|}
\hline
                & Accuracy & Throughput(fps) & Response   efficiency \\ \hline
Tent            & 79.2     & 32.1            & 0.9                   \\ \hline
EcoTTA          & 81.7     & 22.8            & 0.7                   \\ \hline
ElasticTrainer  & 73.4     & 60.6            & 2.1                   \\ \hline
Ours            & 79.5     & 79.4            & 2.6                   \\ \hline
Ours (Adaptive) & 74.8     & 98.8            & 4.4                   \\ \hline
\end{tabular}
}
\label{exp:table_5}
\end{table}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Energy Consumption.}
Although energy consumption is not the primary objective of SwiftTTA optimization, it can significantly reduce the number and length of backpropagations (computational workload), thereby substantially reducing the training energy consumption as a byproduct.

\subsection{Memory Consumption.}








==> body/others/backg_and_motiv.tex <==
%总分总或者总分结构！
\subsection{Model adaptation on mobile device}

%云端训练数据往往无法涵盖所有的移动场景，导致模型在移动端部署后还需要重训练（适应）来维持预测精度。目前移动端的微调模式是离线重训练：预先收集并标注目标部署场景的数据样本，随后进行持续数十个小时的设备端训练【cite melon，et，sage】。然而，标注数据和训练过程非常耗时，这意味着重训练过程只能离线进行，新场景中的推理任务必须等重训练过程结束后才能开始。当移动设备面临的场景频繁切换时，需要不断执行数据标注和重训练过程。此外，在模型部署和推理前就收集到新场景的训练数据可能十分困难甚至不可能，例如在无人机监测任务中，提前一天收集无人机第二天将要部署环境的数据。
Cloud data for training fails to cover all mobile scenarios, resulting in the adaptation of NN model on mobile devices to maintain inference accuracy after deployment. 
The common adaptation mode on mobile devices is offline retraining: pre-collecting and annotating samples from deployment scenarios, followed by offline multi-epoch training on device\cite{} or cloud\cite{}.
However, data annotation and offline retraining are time-consuming\cite{}. So inference tasks in new scenarios must wait to begin until the offline retraining is completed.
When mobile devices frequently encounter different scenes, it has to continually perform data annotation and offline retraining which significantly affects the efficiency of mobile task execution.
In addition, collecting retraining data in new scenarios before NN model deployment is challenging. For example, in tasks such as drone surveillance\cite{} and autonomous driving\cite{}, pre-collecting data in environment where the device will be deployed the next day is impossible.

%测试时适应（TTA），又称为无源域适应（source-free domain adaptation），是域适应领域的一种无监督训练模式。TTA的模式十分适用于连续变化的移动端场景：不需要预先进行任何数据准备和离线训练，仅在真正执行推理任务时基于当前需要推理的数据完成无监督的模型适应。TTA主要包括三个阶段：forward-backward-reforward。在forward和backward阶段，模型基于当前数据完成一轮反向传播。在reforward阶段，完成适应的模型再次对当前数据完成推理。这三个阶段是在模型推理时在线运行的，因此backward和reforward的执行时延直接影响了模型推理移动端数据流的帧率。然而将现有的TTA方法部署在移动设备上时，移动设备有限的算力会产生较高的计算时延，这严重影响了模型推理数据流的效率。此外，测试时适应和离线训练并不冲突，可以耦合使用以进一步提高推理精度：在部署前基于新场景数据集完成通用性离线适应，在执行推理任务时对当前输入样本进行针对性在线适应。
Test-Time Adaptation(TTA)\cite{} is an unsupervised adaptation mode in the field of domain adaptation\cite{}. 
It's worth noting that TTA and offline retraining can be coupled for further improving inference accuracy. 
Generic offline adaptation based on new scenario dataset can be completed before deployment, and targeted online adaptation can be performed on inference data input during tasks execution.
TTA is suitable for dynamic mobile scenarios because TTA don't need data annotation and offline retraining. 
Instead, model adaptation is performed online only based on unsupervised inference data stream when tasks execute.
TTA involves three stages\cite{liang2023comprehensive}: forward, backward, and reforward.
During forward and backward, model completes adaptation with once forward propagation and backward propagation based on inference data input. 
In reforward, adapted model performs inference again on inference data input.
Three stages online execute during inference, so the latency of backward and reforward directly affects the inference efficiency on mobile data stream.
However, as shown in Figure 2-1, deploying existing TTA methods on mobile devices will results in high latency which impacts efficiency of inference due to limited computational capability.


\subsection{Opportunities for TTA Speedup}
%现有的TTA方法致力于解决在连续适应条件下错误累计带来的精度下降问题，部署在资源有限的移动端后可能产生性能问题。我们首先分析这些方法在移动端设备上的适用性。
%一类方法通过减小伪标签对整个模型参数的影响来减轻错误累计问题，这些方法只更新模型的BN层或其他标准化层的参数。但由于反向传播计算具有依赖性，因此适应时延和参与适应的参数量并非正比关系。如图xx（a）所示，尽管只更新第一层参数，但需要反向计算整个网络的梯度，适应时间和更新后四层的四倍参数的时间相同。因此尽管这些方法只更新小部分参数，但依然会导致非常高的适应时延。因为反向传播计算具有依赖性，适应时延和参与适应的参数量并非正比关系。并且只更新少量的标准层参数会影响模型的适应能力，导致适应后精度提升有限~\cite{cotta}。
%另一类方法在适应时通过提高伪标签的可信度来减轻错误累计问题，更可靠的伪标签让这些方法即使更新整个模型的参数也能够保持连续适应后的精度。然而，计算更准确的伪标签会带来额外的计算成本（例如cotta的多个伪标签融合~\cite{cotta}），并且更新整个模型需要完整的反向传播计算。这会导致当这些方法部署在移动设备上时会产生较高的在线适应时延，从而影响模型的推理效率。
%相比于从头训练，模型在移动端部署后的适应是为了微调参数以适应新场景数据和云端训练数据间的分布差异。对于不同类型和程度的分布偏移，不同的层在微调中过程显示出了不同的重要性~\cite{}，只微调最重要的一部分层的精度甚至提升比微调整个模型的精度提升更高。这给在保持微调精度的情况下用模型稀疏更新来加速微调过程带来了时延优化机会。然而在缺乏数据集类型等元信息的真实场景中，实时数据的分布偏移类型和程度是潜在和难以刻画的。因此关键挑战是如何对移动场景t时刻的数据流，实现模型每层对应微调重要性的建模。
%如果进一步考虑更新每层给模型适应带来的时延开销，并权衡精度-时延进行搜索，就能够在实现低时延的同时保持模型适应带来的精度收益。此外，只更新部分参数还能够减轻连续适应带来的错误累计现象。
Existing TTA methods aim to solve accuracy decline caused by error accumulation after continuous unsupervised adaptation. 
So when deployed on resource-constrained mobile devices, they may lead to performance challenges. 
We first analyze the applicability of these methods on mobile devices.


One kind of TTA methods solve error accumulation by reducing the impact of wrong pseudo-labels on model parameters. 
These methods only update parameters of batch normalization(BN) layers\cite{} or other normalization layers\cite{}. 
However, due to the dependency of backpropagation chain, adaptation latency and the number of updating parameters are not directly related. 
As shown in Figure xx (a), even only the first layer parameters are updated, the gradients of entire network still need to be computed, resulting in adaptation latency equal to updating last four layers parameters, even latter involves four times more parameters.
%因此尽管这些方法只更新小部分参数，但依然会导致非常高的适应时延。因为反向传播计算具有依赖性，适应时延和参与适应的参数量并非正比关系。并且只更新少量的标准层参数会影响模型的适应能力，导致适应后精度提升有限~\cite{cotta}。


Another kind of TTA methods addresses error accumulation by enhancing confidence of pseudo-labels~\cite{}. 
More reliable pseudo-labels can maintain accuracy after continuous unsupervised adaptation even updating the parameters of the entire model. 
%然而，计算更准确的伪标签会带来额外的计算成本（例如cotta的多个伪标签融合~\cite{cotta}），并且更新整个模型需要完整的反向传播计算。这会导致当这些方法部署在移动设备上时会产生较高的在线适应时延，从而影响模型的推理效率。

%相比于从头训练，模型在移动端部署后的适应是为了微调参数以适应新场景数据和云端训练数据间的分布差异。对于不同类型和程度的分布偏移，不同的层在微调中过程显示出了不同的重要性~\cite{}，只微调最重要的一部分层的精度甚至提升比微调整个模型的精度提升更高。这给在保持微调精度的情况下用模型稀疏更新来加速微调过程带来了时延优化机会。然而在缺乏数据集类型等元信息的真实场景中，实时数据的分布偏移类型和程度是潜在和难以刻画的。因此关键挑战是如何对移动场景t时刻的数据流，实现模型每层对应微调重要性的建模。
%如果进一步考虑更新每层给模型适应带来的时延开销，并权衡精度-时延进行搜索，就能够在实现低时延的同时保持模型适应带来的精度收益。此外，只更新部分参数还能够减轻连续适应带来的错误累计现象。



\subsection{Sparse Updating in Online Adaptation}
%测试时适应在模型推理时在线运行，复杂且动态的移动端环境、给适应过程带来了两个挑战：动态的硬件环境和数据分布。
TTA runs online during device executes tasks. Compared to offline training conditions, complex and dynamic runtime conditions bring two challenges to online adaptation: dynamic device resources and data distributions.

\textbf{Dynamic device resources.}
\label{Dynamic device resources.}
%稀疏更新方法需要准确的层时延信息以保证搜索得到的更新策略符合预期加速效果。和内存、能耗等指标不同，时延是一个动态性指标，即使在同一个设备上执行同一个操作的时延也会随着设备条件的变化而变化。先前的稀疏更新方法基于离线环境测量的每层时延信息完成重训练时的策略搜索。因为重训练很少与其他计算任务共同执行,因此离线测量环境和重训练环境（通常在深夜）下的时延相差很小\cite{}。然而测试时适应在设备推理时运行（例如白天），这意味着它需要和设备上更多的其他进程同时竞争设备资源，例如无人机的控制程序、手机的应用程序。并且设备的硬件条件如温度也可能发生大幅变化。现有的时延分析方法\cite{}主要预测给定网络结构在黑盒设备理想条件下的执行时延。忽略了运行时动态的设备条件给时延带来的影响。为了让策略实际加速效果符合预期，需要实时分析当前设备条件下每一层准确的时延。
Sparse update requires accurate layer latency estimate to ensure that update strategy can achieve expected acceleration goal.
Latency is a highly dynamic metric and even the latency of the same operation executed on the same device varies with different device resources.
Previous sparse update methods search update strategy based on offline once estimate of layer latency\cite{} and strategy works well during retraining.
Because offline retraining is rarely performed concurrently with other computational tasks(typically executed during night), hardware resources between estimate and retraining are minimal\cite{huang2023elastictrainer}.
However, TTA runs during device executes tasks(typically during the day), which means it needs to share device resources with more other computational processes on device, such as flight control program of a drone or applications of a smartphone. 
Additionally, device hardware conditions such as temperature, may significant changes.
These factors result in significant discrepancies between actual execution latency and offline estimate latency of the same layer.
Existing latency analysis methods\cite{} primarily predict execution latency of a given network structure under offline conditions of a black-box device. 
However, these methods ignore the impact of dynamically changing device conditions on latency during runtime. 
To ensure that actual acceleration goal align with searched strategy expectations, it is necessary to predict actual execution latency of each layer under dynamic device conditions.




\textbf{Dynamic data distribution.}
\label{Dynamic data distribution.}
%稀疏更新方法需要准确的层精度重要性以保证搜索得到的更新策略能实现预期精度提升。模型训练时每层的精度重要性不固定，而是根据新场景数据集与云端数据集间分布的偏移类型和程度而改变[surgical,和它的引文]。TTA环境下实时数据流的分布未知并且实时变化，因此需要对每一批次的数据频繁评估其对应的层精度重要性。先前的稀疏更新策略[ET,256KB]在同分布的微调数据集上完成训练，因此只需要在多轮训练中一次性（离线单层微调[256KB]方法）或定期（基于完整反向传播[ET]的梯度方法）评估层精度重要性。但这些评估的时延成本较高甚至超过训练本身，因此在需要频繁评估的实时数据流条件下，会造成极高的开销，严重影响模型的效率。
Sparse update requires accurate layer accuracy importance to ensure that update strategy can achieve expected adaptation accuracy improvement.
Accuracy importance of each layer during training is not fixed but rather changes based on the type and level of distribution shift between mobile scene data and cloud data\cite{surgical, and its references}.
The distribution of online data stream in TTA is unknown and continuously changing. 
Therefore, it is necessary to frequently estimate layer accuracy importance for online data stream.
Previous sparse update methods\cite{huang2023elastictrainer, lin2022device} focus on offline retraining on independent and identically distributed(IID) fine-tuning dataset. 
Therefore, these methods only execute layer accuracy importance estimation either once (offline single-layer fine-tuning\cite{lin2022device}) or periodically (gradient-based method through complete backward\cite{huang2023elastictrainer}) during multiple training epochs.
However, once execution latency of these evaluation methods is equal to or even exceeds once backward during training, as shown in Figure xx. 
Therefore, frequent evaluations will lead to extremely high latency on online data stream, severely impacting the efficiency of NN model.





%\subsection{Sparse updating for Responsive Adaptation}
%在TTA中，对于一批输入数据，模型需要先完成在线适应后才能给出预测结果。因此模型适应的速度十分重要，直接决定了模型预测的速度，特别是在无人机监测等对时延要求较高的场景中。然而，目前的TTA方法聚焦于提高无监督训练的可信度和训练精度，并面向服务器设备展开设计和验证。当这些TTA方法部署在资源有限的移动端设备时，会造成较高的适应时延，严重影响了设备端任务预测的速度。最近，XX等人提出了第一个内存高效的on-device TTA方法——EcoTTA，which通过避免存储主干网络的中间激活来减少内存消耗。然而，EcoTTA在部署时依然会面临高时延的挑战，如图xx所示\cite{}。
%稀疏更新技术通过稀疏化模型训练时延的bottleneck——反向传播计算，来加快模型训练的速度或减少训练内存占用。在调研了设备端训练加速技术后，我们发现稀疏更新是加速测试时适应的理想技术。第一，在无监督训练中，伪标签带来的可能性错误监督会导致模型在多轮适应后的精度不断下降甚至崩塌，叫做错误累计现象。为了应对错误累计，TTA方法通常只更新模型的一部分参数，例如BN层【cite：tent，eata】，来减轻累计错误对模型的影响。因此稀疏更新有机会同时解决适应时延问题和错误累计问题。第二，稀疏更新能够通过控制反向传播的稀疏程度实现对适应速度快慢的动态调整，这在预测数据流等对帧率有灵活要求的任务中尤其重要。其他技术例如计算卸载技术在缺少DSP等结构的设备上难以适用，量化技术带来的精度损失会在无监督适应中进一步放大。但如果需要进一步加速，稀疏更新技术作为一种更新模式，能够方便地和这些技术耦合使用。


==> body/others/background_v2.tex <==
%由于位置和时间变化，移动设备例如手机、虚拟/增强现实 (VR/AR) 耳机、机器人、车辆和智能电器通常需要在non-stationary的环境下执行深度学习数据流推理任务，这为on-device task的输入数据带来了高variability。
%Examples include 
%(1)A vision sensor system of an autonomous vehicle can be exposed not only to fog, snow, and rain, but also to rare conditions including smoke, sand storms, or substances distributed on the road in consequence of a traffic accident. 
%当汽车行驶时，不同地点和天气会给on-device语义分割任务带来输入街景数据的潜在分布差异。
%例如城区和乡下，不同城市会带来道路类型，建筑风格，拍摄角度的差异。
%不同天气包括night，fog, snow, and rain，特殊环境including smoke, sand storms，会影响光照、对比度和物体遮挡情况。
%此外，还可能收集到corrupted images resulting from sensor degradation。
%(2)随着用户位置和视角的不断变化，AR headset需要不断学习来识别视野中的相关物体和区域，以适当定位虚拟感知信息。
%(3)Household robotic devices need to learn the identity of the individuals, pets, and objects in the house. Changes in user requirements and environment such as from daylight to nightlight

%根据以上示例，我们认为这些功能对于on-device adaptation系统至关重要： 
%1.在资源受限的环境中在线完成学习并及时给出学习后的推理结果。 
%2.不对连续数据流的分布作出任何假设。数据流的分布是未知、不稳定和难以预测的。  
%3.使用缺少标签的实时数据流进行有效的在线学习和推理。

%这些标准可以概括为：我们需要在连续变化和不稳定的实时数据流without labels下完成on-device在线学习和推理。

%%%%%%%%%%%%%%%%%%%%%正文%%%%%%%%%%%%%%%%%%%%%%%%

%motivation的论述
\section{Background}
\label{sec:background}

\subsection{Why Test-time Adaptation}
\label{sec:background:why}

\subsubsection{Primer on Test-time Adaptation}
\zimu{Test-time adaptation (TTA) is an emerging \textit{unsupervised domain adaptation} paradigm to combat \textit{domain shifts} \cite{liang2023comprehensive}.
It adapts the model parameters \textit{pre-trained} in the source domain to \textit{unlabelled} target data during \textit{testing}, aiming to enhance the inference accuracy on the target data \cite{wang2020tent}.
Uniquely, TTA assumes no access to the \textit{source data} and \textit{supervision} from the pre-training stage, which distinguishes itself from supervised training \cite{wang2022melon, gim2022memory, huang2023elastictrainer}, transfer learning \TODO{refs}, generic domain adaptation \cite{taufique2021conda, tang2021gradient}, \etc
This setup is advantageous in mobile applications where \textit{(i)} accessing source data is impractical due to privacy concerns or bandwidth limitations; and \textit{(ii)} annotating the target domain data is infeasible or labour-intensive \cite{wang2020tent, wang2022continual, niu2022efficient, song2023ecotta, hong2023mecta}.
A more comprehensive comparison with relevant paradigms is deferred to \secref{sec:related}.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%tta是一种特殊的domain adaptation技术，致力于解决由训练时source data和测试时target data间存在的分布差异而带来的模型在测试环境下推理精度下降的问题。
%tta使用基于source data预训练的模型和没有标签的target data完成模型参数对target data分布的适应，以提高在target data上test的精度。
%相比origin DA在适应时通常需要同时访问来自源域的标记数据和来自目标域的(未标记的)数据,tta在适应时不需要访问来自源域的数据、特征或标签，这在医疗数据等隐私敏感的移动应用中尤为重要。

% \fc{
% Test-time adaptation is a special domain adaptation technique which aims to address DNN model decreased inference accuracy in test environments due to distribution differences between source data during training and target data during test.
% %
% Test-time adaptation utilizes the model pre-trained on source data and unlabeled target data from test environment to adapt the model parameters to the distribution of target data, improving the inference accuracy on target data.}
% %

% \fc{
% Compared to efficient supervised training~\cite{wang2022melon, gim2022memory, huang2023elastictrainer} and continual on-device adaptation~\cite{ma2023cost,pellegrini2020latent,demosthenous2021continual}, test-time adaptation finishes model adaptation only based on unlabeled target data, thus avoiding the costly and latency-consuming process of target data annotation, enabling higher adaptation efficiency.
% Compared to continual domain adaptation~\cite{taufique2021conda,tang2021gradient}, which typically requires accessing labeled source data and unlabeled target data during adaptation, test-time adaptation does not need to access data, features, or labels from the source domain during adaptation, which is particularly crucial in mobile applications such as medical data because of limited transmission bandwidth and strict privacy protocols.
% }

%One kind of previous studies usually use offline retraining~\cite{wang2022melon, gim2022memory} or continual on-device adaptation~\cite{ma2023cost,pellegrini2020latent,demosthenous2021continual} techniques to adapt model in the mobile scene which requires data collecting and manual data labeling.(Figure~\ref{fig:offline_tta_chameleon} (A)).
%When deployed in non-stationary and continually changing mobile environments, manual data labeling with significant time cost will limit the efficiency of model adaptation and these methods cannot adapt to new environment rapidly.
%持续域适应
%The other kind of studies use continual domain adaptation~\cite{taufique2021conda,tang2021gradient} to adapt DNN model.
%Continual domain adaptation can adapt directly based on unlabeled data without data labeling, however, it requires the access to a large amount of source data stored in cloud, which is difficult in mobile with limited transmission bandwidth and strict privacy protocols.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Our Scope}
%介绍tta for nonstationary environments（特殊类型的online small batch tta）
%我们是在一个small batch上做online adaptation。强调我们具体是哪一种类型tta，以及为什么（nonstationary环境带来一些数据特性）（这些数据和标签的特性导致我们需要做这样的tta）
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We explore TTA for \textit{responsive} adaptation to \textit{non-stationary} domain shifts, which corresponds to the following requirements.
\begin{itemize}
    \item \textbf{Low Latency}.
    \item \textbf{Small Batch}.
\end{itemize}




\sysname is based on online test-time adaptation mode with small batches, which can adapt to continually changing and non-stationary environments.
The existing test-time adaptation can be categorized into three modes: source-free domain adaptation, test-time batch adaptation, and online test-time adaptation.
The first two modes belong to offline test-time adaptation, and their applicability is limited in continually changing and non-stationary environments.
Because source-free domain adaptation typically requires collecting a certain number of samples from new environments in advance and completing offline model adaptation, which may be infeasible for streaming data scenarios where unknown and unpredictable data arrives continually and in sequence.
Moreover, offline test-time adaptation is one-time adaptation, requiring constant resetting of the model's original parameters after adaptation to continually readjust to later arriving data in continuous scenarios, which will decrease the efficiency and accuracy of continually model adaptation.

%SOURCE-FREE DOMAIN ADAPTATION需要提前收集大量新场景的数据并完成离线模型适应。但the distribution of continuous data streams which is unknown, unstable, and difficult to predict.新场景数据难以提前预测和收集。
%TEST-TIME BATCH ADAPTATION能够基于更少量的数据（通常是一个批次甚至一张样本）完成适应。但这种适应是一次性的，在连续场景下TEST-TIME BATCH ADAPTATION需要不断在适应后恢复模型参数以重新适应新到达的数据，这会降低模型适应的效率和精度。
%\sysname 是一种online tta技术based on small batches which 能够应对continually changing and non-stationary环境。（借鉴综述对online的描写）
%现有的tta主要分为三种模式，SOURCE-FREE DOMAIN ADAPTATION，TEST-TIME BATCH ADAPTATION 和 ONLINE TEST-TIME ADAPTATION。
%前两种模式是offline tta，在continually changing and non-stationary环境下的适用性有限。
%因为SOURCE-FREE DOMAIN ADAPTATION通常需要提前收集一定规模新场景的数据并完成离线模型适应，这对于数据连续且按顺序到达的流数据场景来说可能是不可行的。
%并且offline tta是一次性适应，在连续场景下需要不断在适应后恢复模型原始参数以重新适应新到达的数据，这会降低连续模型适应的效率和精度。
%online tta在测试期间模型面临新数据时即时触发模型适应which能够较好地应对实时数据流，并且能够重用在线学习等过去的知识，实现持续的适应而无需每次适应后重置模型参数。
%此外，由于需要基于实时数据流完成适应和推理，因此每次数据收集窗口较短，难以形成较大批次。\sysname通常需要基于小批次数据完成在线适应。
% \fc{
% \sysname is based on online test-time adaptation mode with small batches, which can adapt to continually changing and non-stationary environments.
% The existing test-time adaptation can be categorized into three modes: source-free domain adaptation, test-time batch adaptation, and online test-time adaptation.
% The first two modes belong to offline test-time adaptation, and their applicability is limited in continually changing and non-stationary environments.
% Because source-free domain adaptation typically requires collecting a certain number of samples from new environments in advance and completing offline model adaptation, which may be infeasible for streaming data scenarios where unknown and unpredictable data arrives continually and in sequence.
% Moreover, offline test-time adaptation is one-time adaptation, requiring constant resetting of the model's original parameters after adaptation to continually readjust to later arriving data in continuous scenarios, which will decrease the efficiency and accuracy of continually model adaptation.
% }


%1、不能提前收集
%2、需要在连续的data batches上不断适应

%在线适应能够在模型面临新数据时即时触发适应过程，并在适应后返回推理结果。

%随着移动设备的不断moving，on-device deployed DNN model面临continually changing and non-stationary环境。
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Example Applications}
%为了强调我们的这种tta是有意义的，里边放一些特性，比如source-free、nonstationary什么的
\TODO{two examples}
%在真实移动场景下，on-device deployed DNN model经常面临continually changing and non-stationary环境。
\fc{
In real mobile applications, on-device deployed DNN models often encounter continually changing and non-stationary environments.
%
(1)Different locations and weathers affect the potential distribution of the input street scene data for autonomous driving tasks as the car moves.
Specifically, road types, architectural styles, and shooting angles will differ from urban and rural areas, as well as among different neighborhoods.
Different weathers such as night, fog, snow, and rain, as well as rare conditions like smoke and sandstorms, will affect illumination, contrast, and object occlusion in collected data.
Additionally, sensor degradation may also result in different degrees of corrupted images.
(2)AR headsets need to continually learn to identify relevant objects and regions in the field of view to appropriately position virtual perceptual information as the user's position and perspective constantly change.
(3)Household robotic devices need to learn the multi-view identity of the individuals, pets, and objects in dynamic user requirements and changing environments such as from daylight to nightlight.
}
\lsc{It is necessary to update on-device DNNs in real-time, to promptly online adapt to the new live data distributions or real-time feedback from the environment.}





\subsection{Latency of Test-time Adaptation}
\label{sec:background:latency}

\subsubsection{\fc{Latency Breakdown}}
%需要强化一下我们的the forward, backward, re-forward workflow三个stage，和正常的forward和backward是不太一样的
\TODO{highlight the forward, backward, re-forward workflow, so that we differ from standard on-device training, and from some special evaluation protocols of online TTA}

\fc{
Compared with the standard live data inference process, test-time adaptation adds the process of online \textit{backward} and \textit{reforward}. 
Therefore, optimizing the latency of backward and reforward is crucial to improve the throughput (fps) of streaming data inference. 
Although existing online test-time adaptation methods can improve model inference accuracy, limited computational resources in mobile devices will lead to high adaptation latency.\TODO{add a comparison table}
In our study, we aim to optimize the delay of test-time adaptation process to further improve the availability of test-time adaptation in mobile scenarios, as shown in~\ref{fig:offline_tta_chameleon} (C).
Due to the special evaluation protocol and the running condition of online device, the latency components and variation of online test-time adaptation differ significantly from offline on-device training.
First, due to the evaluation protocol of online test-time adaptation requiring reporting of forward accuracy after adaptation\cite{liang2023comprehensive}, online test-time adaptation involves different adaptation stages and latency components.
Different with standard on-device training and some special continual test-time adaptation methods which only perform adaptation(including forward and backward) stage, \sysname includes adaptation(forward and backward) and re-evaluation(reforward) stages, which reports forward prediction accuracy after adaptation stage to reflect the accuracy benefits brought by adaptation stage.
Second, adaptation latency in dynamic resource condition during device running is significantly different with offline analyzed latency in static resource condition. 
}


%To achieve the expected latency acceleration, it is necessary to predict the actual execution latency based on offline latency and real-time device resource parameters. 
%Therefore, our final optimizing goal, as Eq.~\ref{search_target},

%加一个表，展示现有tta技术的引入尽管能够提高推理精度，但会大幅降低推理的效率
%由于在线适应和模型推理顺序执行，因此online tta是时延敏感的
% 因此，合理的分配计算资源可以更有效的提高TTA的时间效率。
%Therefore, selectively updating only important DNN model parts can improve the time efficiency of test-time adaptation.
% 在我们的研究中，我们的目标为优化TTA过程的时延，以进一步提高TTA在移动场景中的可用性，如图\ref{fig:offline_tta_chameleon} (C)所示。

\fc{
To reduce the latency of online test-time adaptation, we first analyze the time overhead of online test-time adaptation in mobile environments.
The adaptation stage including once forward and backward propagation based on input data.
In re-evaluation stage, the model performs another forward propagation to generate the prediction based on optimized model.
Therefore, the online test-time adaptation latency can be represented by Eq.~\ref{d1},
\begin{equation} \label{d1}
\begin{aligned}
\lsc{T_{dyn}=T_{u_{dyn}}+T_{re_{dyn}}=T_{f_{dyn}}+T_{b_{dyn}}+T_{re_{dyn}}}
\end{aligned} 
\end{equation}
%式中$T_{u}$为模型适应的延迟时间，包括$T_{f}$和$T_{b}$两个分量，分别为正向和向后的延迟时间。$T_{i}$是重新推理的延迟时间。
where $T_{u_{dyn}}$ is the latency for DNN updating and $T_{re_{dyn}}$ is the latency of reforward. 
$T_{u_{dyn}}$ includes two components $T_{f_{dyn}}$ and $T_{b_{dyn}}$, which are the latency of forward and backward respectively.
}




\subsubsection{Latency Bottleneck}
\TODO{show through measurements that backward is the bottleneck}
\fc{We further analyze the bottleneck of online test-time adaptation latency to decrease $T_{dyn}$.
As shown in Figure~\ref{fig:forward_backward_latency}, we observe that the backward propagation latency, $T_{b_{dyn}}$, is much larger than the forward latency, $T_{f_{dyn}}$ and $T_{re_{dyn}}$, in test-time adaptations for different network architectures on mobile. 
The latency due to backward propagation is more than 50\% even 60\% in all networks, much more than the other parts.}
\begin{figure}
  \centering
  \includegraphics[width=0.9\linewidth]{figure/forward_backward_latency.pdf}
  \caption{Latency components of test-time adaptation with three typical DNNs on Nvidia Jetson NX.}
  \label{fig:forward_backward_latency}
\end{figure}
\fc{
To optimize the adaptation efficiency, we further analyze the primary factors affecting the latency of backward propagation.
Specifically, in forward propagation, the model only needs to compute the forward output of each layer, as in Eq.~\ref{e1},
\begin{equation} \label{e1}
T_{f_{dyn}} = T_{re_{dyn}} = \sum_{l=1}^L{T_{l,f}^{dyn}},
\end{equation}
where $l \in [1,L] $ is the number of layers in whole network and 
$T_{f_{dyn}}$, $T_{re_{dyn}}$ is the forward and reforward latency of layer $l$, respectively.
However, in backward propagation, the latency of each layer mainly comes from the gradient computation of the parameters $\sigma_l$ and input $x_l$ at each layer, as shown in Fig. \ref{fig:latency_formulation_of_layer_i_}.
}

\fc{
Therefore, the backward propagation latency can be presented as:
\begin{equation} \label{e2}
T_{b_{dyn}}=\sum_{l=1}^L{T_{l,b}^{dyn}}
\end{equation}
where $t_a(\frac{\partial t}{\partial \sigma_l}, x_l)$ is $l$ the latency of gradient calculation, $t_b(\sigma_l)$ is latency in other procedures of back propagation.
The more complex gradient calculations bring greater computational latency for backpropagation than forward.
Therefore, optimizing the key to online test-time adaptation is to optimize the gradient computation latency of backpropagation stage.
}


\begin{figure}[t]
  \centering
  \includegraphics[width=0.48\textwidth]{figure/latency_formulation_of_layer_i_.pdf}
  \caption{Latency formulation for layer $i$ }
  \label{fig:latency_formulation_of_layer_i_}
\end{figure}

\subsection{Opportunities and Challenges}
\label{sec:background:problem}

\subsubsection{Opportunities}
\TODO{state partial update as the opportunity here, and move the formal problem definition here}

%我们发现xx技术
%1、从时延方面，当前的full updating很花时间
%更新少的层带来更少时延
%一些稀疏更新技术并不时延高效，因为xxx（已有段落）
%2、从精度方面，更新更少重要的层并不会损害精度
%而现有的稀疏更新更新固定层（BN）的精度提升有限，因为已有研究表明层重要性随着数据分布变化而改变。
%因此在实时连续变化的不稳定场景下，频繁评估能够选择更重要的层，从而提升适应精度
%从这两个方面来看，需要选择一个最优的策略，包含的层能够在满足时延约束目标的情况下具有最大的精度收益

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fc{
We observe that sparse updating methods which only update DNN important layers provide an opportunity to reduce online test-time adaptation latency while keep maintaining adaptation accuracy.
(1)Lower adaptation latency. 
According to Eq.\ref{e2}, fully computing gradients for all layers leads to high latency.
Therefore, skipping gradient computation of a part of DNN layers is an effective way to reduce the backpropagation latency.
However, some sparse updating methods (e.g. BN-based) only update xx\% of parameters, yet they only caused a lower than xx\% latency reduction because updating fewer layers may not result in a corresponding decrease in adaptation latency.
As shown in Figure~\ref{fig:layernum_latency}, the backward latency for updating the first layer is the same as the latency for updating the last four layers.
Because the updating of each layer depends on the gradient of the current layer in the backward stage, we need to calculate the gradient of all previous layers to get the final result of the current layer.
Therefore, we need to consider not only the number of optimized updating layers but also the location of updating layers.
(2)Comparable adaptation accuracy. 
Existing research shows that only updating important layers even can get higher accuracy than the entire model as it reduces model overfitting issues during adaptation~\cite{evci2022head2toe, lee2022surgical}.
However, existing sparse updating methods which update fixed important layers\cite{wang2020tent,niu2022efficient} or periodically adjusting the importance of layers\cite{huang2023elastictrainer} results in limit accuracy improvements in continually changing and non-stationary environments because previous research has shown that the importance of each layer changes as input data distribution changing and online layer importance could be largely different in different environments, leading to noticeable accuracy loss.
Continually and frequently selecting the most important layers based on the streaming input data from non-stationary environments allows timely adaptation to data distribution changing in real-time to improve adaptation accuracy.
Therefore, it is necessary to consider both adaptation latency and accuracy and select the optimal sparse update strategy which ensures that the layers chosen for update achieve maximum accuracy gains while satisfying latency constraints.
}
\fc{
\sysname aims to maximize the accuracy of online test-time adaptation under given latency requirement in non-stationary and continually changing mobile environments through layer-wise sparse updating. 
Under the environment $e$, the design goal is formulated as a constrained optimization problem as follows:
\begin{equation} \label{search_target}
    \max\text{\,\,}\vec{S}_e\cdot \vec{A}_e\,\,\,\,\,\,\,s.t.\,\,\,T_{f_{dyn}}+T_{b_{dyn}}^{'}\left( \vec{S}_e \right) +T_{re_{dyn}}^{'}\left( \vec{S}_e \right) \le \sigma \cdot T_{dyn}
\end{equation}
where $\vec{S}_e$ is sparse updating strategy, $\vec{A}_e$ is layer importance vector, $T_{b_{dyn}}^{'}$ and $T_{re_{dyn}}^{'}$ is optimized backward latency and reforward latency under strategy $\vec{S}_e$, $T_{dyn}$ is fully updating latency and $\sigma$ is expected acceleration factor of training latency according to mobile task requirement.% $F_{e}$: $T_e=\frac{1}{F_e}$. 
Within a inference task like object detection, the expected acceleration factor $\sigma$ is usually dynamically adjusted by the app or user at runtime.
}

\begin{figure}[t]
  \centering
  \includegraphics[width=.83\linewidth]{figure/layernum_latency.pdf}
  \caption{Example of Latency in Updating. GC means gradient calculation. Both updating one layer and updating four layers result in the same GC computation latency.}
  \label{fig:layernum_latency}
\end{figure}


\subsubsection{Challenges}
\TODO{to be better aligned with the solution, I think the first challenge should be something related to efficient layer importance assessment, not data-dependent}
\TODO{the 3rd challenge is vague}


%尽管通过改变层的更新可以加速TTA，但如何在移动场景构建层的更新策略同样是一个挑战。
\fc{
While online test-time adaptation can be accelerated by sparse updating, how to search important updating layers precisely and efficiently based on streaming data changing real-time is a key challenge.
We need to consider the following challenges brought by non-stationary and continually changing environments:
}
\begin{itemize}
    
    \item \fc{\textbf{Backward-free layer importance assessment} %解决两个层重要性评估中的挑战，一个是rely data label（unsupervised），一个是high latency（real-time）
    Layer importance needs frequent assessment and update to adapt to real-time changing streaming data distribution as mobile environment changes.
    The previous methods relies on backpropagation with \textbf{data label requirement} and \textbf{high latency} to assess layer importance~\cite{huang2023elastictrainer,lin2022device} which significantly decrease the efficiency and accuracy of frequent layer importance assessment in online test-time adaptation.
    }
    \item \fc{\textbf{Resource-aware layer updating latency profiling} 
    High variability of available device resources in online test-time adaptation leads to significant difference between the runtime latency and offline measurement latency of each layer.
    Existing latency measurement methods based on static resource condition may result in sparse update strategies that are difficult to achieve the expected latency optimization goal under dynamic resource conditions.
    }    
    \item \fc{\textbf{Online layer update scheduling} 
    Due to additional reforward stage of online test-time adaptation, modeling the expected adaptation latency of updating selected layers for searching is a key challenge.
    Moreover, since Eq.\ref{search_target} is a non-linear integer programming NP-hard problem, searching for the most important layers to update under expected adaptation latency will incur significant search latency for latency-sensitive adaptation.
    }
\end{itemize}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Time Bottleneck on Test-time Adaptation}
\subsection{Time-efficient On-device Adaptation}
% 云端的训练数据通常无法包含所有实际移动场景的情形，因此在实际部署移动设备时，移动设备无法到达预期的精度。
Training data in cloud often does not include all mobile scenarios~\cite{hayes2022online,hong2023mecta,kwon2021exploring}, when the mobile device is practically deployed, the mobile device cannot achieve the expected accuracy~\cite{bhardwaj2022ekya,mirza2023actmad}.
% 因此，为了提升移动端模型的精度，深度模型需要不断适应当前场景~\cite{wang2022continual}。
Therefore, to improve the accuracy of mobile models, models need to continually adapt to the non-stationary environment~\cite{wang2022continual}.

Mobile devices such as smartphones, virtual/augmented reality (VR/AR) headsets, robots and vehicles often need to execute inference tasks such as image classification\cite{rawat2017deep}, object detection\cite{zhao2019object} and semantic segmentation\cite{guo2018review} in dynamic environments which brings high variability to input data stream.
Examples include 
(1)Different locations and weathers affect potential distribution of the input street scene data for autonomous driving tasks as the car moves.
Specifically, road types, architectural styles and shooting angles will differ from urban and rural areas, as well as among different neighborhoods.
Different weathers such as night, fog, snow and rain, as well as rare conditions like smoke and sandstorms, will affect illumination, contrast, and object occlusion in collected data.
Additionally, sensor degradation may also result in different degrees of corrupted images.
(2)AR headsets need to continually learn to identify relevant objects and regions in the field of view to appropriately position virtual perceptual information as the user's position and perspective constantly change.
(3)Household robotic devices need to learn the multi-view identity of the individuals, pets, and objects in dynamic user requirements and changing environments such as from daylight to nightlight.
Based on the examples, we argue the following capabilities are essential for on-device adaptation systems:
(1)Timely and responsive adaptation and inference in resource-constrained environments.
(2)Making no assumptions about the distribution of continuous data streams which is unknown, unstable, and difficult to predict.
(3)Effective adaptation and inference only using real-time collected data streams without labels and source data.
These criteria can be summarized as stating that we need effective on-device online adaptation on continually changing and non-stationary data streams without labels.

% 在先前的研究中，一种方法是离线再训练\cite{wang2022melon,gim2022memory} (在图\ref{fig:offline_tta_chameleon} (A))。该方法首先需要手动采集移动场景中的实际数据进行适应性训练。
%离线训练和持续适应
One kind of previous studies usually use offline retraining~\cite{wang2022melon, gim2022memory} or continual on-device adaptation~\cite{ma2023cost,pellegrini2020latent,demosthenous2021continual} techniques to adapt model in the mobile scene which requires data collecting and manual data labeling.(Figure~\ref{fig:offline_tta_chameleon} (A)).
When deployed in non-stationary and continually changing mobile environments, manual data labeling with significant time cost will limit the efficiency of model adaptation and these methods cannot adapt to new environment rapidly.
%持续域适应
The other kind of studies use continual domain adaptation~\cite{taufique2021conda,tang2021gradient} to adapt DNN model.
Continual domain adaptation can adapt directly based on unlabeled data without data labeling, however, it requires the access to a large amount of source data stored in cloud, which is difficult in mobile with limited transmission bandwidth and strict privacy protocols.

% 为了解决上述的问题，另一种策略是测试时自适应(test-time adaptation) (Figure~\ref{fig:offline_tta_chameleon} (B))，也称为无源域自适应。
To solve the above problems, one optimal strategy is test-time adaptation (test-time adaptation)~\cite{chen2022contrastive,zhang2023domainadaptor}, also called source-free domain adaption~\cite{} (Figure~\ref{fig:offline_tta_chameleon} (B)).
% 这种方法可以摆脱标签的依赖，这避免了人工数据处理时间成本~\cite{liang2023comprehensive}。
This approach is free from target data labels and source data, which avoids the cost of manual data labeling time and privacy issues.
% 同时，由于TTA只需要在移动端自适应，这意味着它有效地克服了模型重部署的时间延迟。
Meanwhile, since test-time adaptation only requires adaptation on device, it also effectively overcomes the latency of redeployment.
% 虽然现有的TTA方法降低了自适应时候移动设备时延。
%Although the existing test-time adaptation method reduces the adaptive time delay of mobile devices. 
% 然而，由于移动场景下计算资源有限，计算资源的无差别分配会导致网络更新的时间效率的降低。
However, due to the limited computational resources in mobile device, the undifferentiated updating of the whole DNN model leads to the decrease of time efficiency of mdoel adaptation.
% 因此，合理的分配计算资源可以更有效的提高TTA的时间效率。
Therefore, selectively updating only important DNN model parts can improve the time efficiency of test-time adaptation.
% 在我们的研究中，我们的目标为优化TTA过程的时延，以进一步提高TTA在移动场景中的可用性，如图\ref{fig:offline_tta_chameleon} (C)所示。
In our study, we aim to optimize the delay of test-time adaptation process to further improve the availability of test-time adaptation in mobile scenarios, as shown in~\ref{fig:offline_tta_chameleon} (C).

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figure/offline_tta_chameleon.pdf}
  \caption{Time bottleneck on different adaptation methods. (A) is offline retraining~\cite{}, it takes more time to collect and annotate new scenario data and retrain the model offline. (B) is existing test-time adaptation methods~\cite{}, it avoids the latency of data collection and labeling and also reduces the time-consuming by online adaptation. (C) is our proposed method, AdaFlow, we further optimize the adaptation and inference process of test-time adaptation to improve model time efficiency in mobile scenarios.}
  \label{fig:offline_tta_chameleon}
\end{figure}



% 在本文中，我们旨在优化TTA过程的延迟，以进一步提高TTA在移动场景中的使用，如图\ref{fig:offline_tta_chameleon} (C)所示。

% The training data from the cloud cannot include all practical scenarios, which often leads to a significant target domain difference on mobile devices. Subsequently, the network accuracy is decreasing dramatically~\cite{bhardwaj2022ekya,mirza2023actmad}.

% To solve this problem, the deployed DNN model needs to continually adapt to the current scenario~\cite{wang2022continual}.

% A preliminary method for mobile data adaption is offline retraining~\cite{wang2022melon,gim2022memory}, as Fig.~\ref{fig:offline_tta_chameleon} (A). However, this approach is subject to two inevitable problems. Firstly, due to the lack of labels, considerable time is required for labeling before training. Secondly, the training process is also quite time-consuming. Obviously, given the time-consuming of offline retraining, it's clearly not ideal for mobile devices. Another option is Test-Time Adaptation (test-time adaptation), also known as source-free domain adaptation. Since test-time adaptation is label-free, this avoids the time overhead of data labeling~\cite{liang2023comprehensive}. Besides, test-time adaptation is exclusively adaptive on mobile, which implies that it effectively overcomes the time latency of model redeployment.
% !!! 这里需要用示意图来表达这三个范式的时延差异，凸显你的是最优的

% Existing test-time adaptation methods have reduced latency to some extent. However, due to computational resource constraints on mobile devices, these approaches still incur large time latency for dynamic mobile scenarios, as Fig.~\ref{fig:offline_tta_chameleon} (B). Therefore, how to improve time efficiency on test-time adaptation-based mobile data adaptation is worth exploring. In this paper, we aim to optimize the latency of the test-time adaptation process to further improve the usage of test-time adaptation in mobile scenarios, as Fig.~\ref{fig:offline_tta_chameleon} (C).
%在本文中，我们致力于在移动场景下对TTA的过程进行时延优化，进一步提高TTA在移动场景的使用率。
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{figure/offline_tta_chameleon.pdf}
%   %\caption{TItle. + 这个图说明的是什么}
%   %\caption{Time bottleneck on different adaption methods. (A) is offline retraining, it 需要数小时收集和标注新场景数据并执行多轮训练. (B) is existing test-time adaptation methods, it 在推理前单次适应，这会产生较高时延，影响推理效率 (C) is Ours, 通过稀疏更新和跨层技术co-design同时优化了适应时延和推理时延. these indicate XXX}
%   %\caption{Time bottleneck on different adaption methods. (A) is offline retraining, it takes more extra hours to collect and annotate new scenario data and also retrains the model for multiple epochs. (B) is existing test-time adaptation methods, 他避免了人工收集和标注数据，并仅通过单次适应，减少时延 (C) is Ours, 进一步优化了TTA的适应和推理过程，进一步提高移动场景下的时间效率。}
%   \caption{Time bottleneck on different adaption methods. (A) is offline retraining, it takes more extra hours to collect and annotate new scenario data and also retrains the model for multiple epochs. (B) indicates existing test-time adaptation methods, they avoid the process of data collection and labeling and also reduce the latency by one-epoch adaptation. (C) is Ours, our approach further optimizes the adaptation and inference process of test-time adaptation to improve model time efficiency in mobile scenarios.}
%   %\caption{离线retraining、现有TTA方法和Chameleon中模型适应的时延对比。}
%   \label{fig:offline_tta_chameleon}
% \end{figure}


% The training data from the cloud cannot include all deployed scenarios, which often leads to a significant data distribution shift between cloud and mobile. Subsequently, the network accuracy is decreasing dramatically~\cite{}. To solve this problem, the model deployed to mobile needs to continually adapt to the current scenario~\cite{}.
% A preliminary method for mobile data adaption is offline retraining~\cite{}. However, this approach is subject to two inevitable problems. Firstly, due to the lack of labels, considerable time is required for labeling before training. Secondly, the training process is also quite time-consuming (several hours~\cite{}). Obviously, given the time-consuming of offline retraining, it's clearly not ideal for continuous changing mobile scenarios. Another option is Test-Time Adaptation (test-time adaptation), also known as source-free domain adaptation~\cite{}. Since test-time adaptation is label-free, this avoids the time overhead of data labeling~\cite{}. 
% Besides, test-time adaptation executes adaptation during model online inference, effectively overcoming the time latency caused by offline training and redeployment.
% % !!! 这里需要用示意图来表达这三个范式的时延差异，凸显你的是最优的

% While test-time adaptation avoids the latency of data annotation and offline training redeployment, it provides inference results for current data input only after the model completes online adaptation. Therefore, the latency of online adaptation directly affects the efficiency of model inference.
% Due to computational resource constraints on mobile devices, existing test-time adaptation methods still incur large time latency in dynamic mobile scenarios, as Fig.~\ref{}. Therefore, how to improve time efficiency on test-time adaptation-based mobile data adaptation is worth further exploration.

%原理级别的论述
\subsection{Opportunities for Time-efficient test-time adaptation}
% 为了降低移动场景下TTA的时延，我们首先分析了移动场景下TTA的时间开销。
To reduce the latency of test-time adaptation, we first analyze the time overhead of test-time adaptation in mobile environments.
% TTA的过程主要包括几个流程。首先进行是适应训练，这主要是网络进行单轮前向传播和模型更新过程。
The process of test-time adaptation mainly consists of two stages~\cite{}. 
The first stage is model adaptation with once forward and backward propagation based on current input data.
% 之后，模型再次经过正向推理，得到最终适应之后的结果。
In the second stage, the model performs reforward inference to generate the final prediction.
% 因此，TTA时延可以由一下表示，如Eq.~\ref{d1}.
Therefore, the test-time adaptation delay can be represented by Eq.~\ref{d1},
\begin{equation} \label{d1}
\begin{aligned}
     \lsc{T} & \lsc{= T_{u} +T_{re} = T_{f}+T_{b}+T_{re}}
\end{aligned} 
\end{equation}
%式中$T_{u}$为模型适应的延迟时间，包括$T_{f}$和$T_{b}$两个分量，分别为正向和向后的延迟时间。$T_{i}$是重新推理的延迟时间。
where $T_{u}$ is the latency for DNN updating and $T_{re}$ is the latency of reforward. 
$T_{u}$ includes two components $T_{f}$ and $T_{b}$, which are the latency of forward and backward respectively.


%我们的目标是降低时延$T$，但是在整个TTA过程中的不同时期，网络时延存在较大的差异。%因此，我们进一步分析了各部分网络时延的占比。
There are large differences between the three components in Eq.~\ref{d1}, we further analyze the bottleneck of test-time adaptation latency to decrease total latency $T$.
%如图~\cite{fig:forward_backward_latency}所示，我们观察到在移动端不同常见的不同网络结构的测试时适应中，后向传播的延迟比前向的延迟要大得多。
As shown in Figure~\ref{fig:forward_backward_latency}, we observe that the backward propagation latency, $T_b$, is much larger than the forward latency, $T_{f}$ and $T_{i}$, in test-time adaptations for common-used different network architectures on mobile. The latency due to backward propagation is more than 50\% even 60\% in all networks, much more than the other parts.
\begin{figure}
  \centering
  \includegraphics[width=0.9\linewidth]{figure/forward_backward_latency.pdf}
  \caption{Latency components of test-time adaptation with three typical DNN architectures on Nvidia Jetson NX.}
  \label{fig:forward_backward_latency}
\end{figure}

To optimize the adaptation efficiency, we further analyze the primary factors affecting the latency of forward and backward propagation.

%具体来说，在前向传播，模型只需要依次计算每层的前向输出，如式\ref{d3}，
Specifically, in forward propagation, the model only needs to compute the forward output of each layer, as in Eq.~\ref{e1},
\begin{equation} \label{e1}
T_{f} = T_{i} = \sum_{l=1}^L{t(x_l,\sigma_l)},
\end{equation}
where $l \in [1,L] $ is the number of layers in whole network and $t(l)$ is the latency in layer $l$ and its parameter $\sigma_l$.

%但是，在后向传播时，各层的延迟主要来自于各层参数$\sigma_l$和输入$x_l$的偏导，也就是梯度计算，此外也包括模型的更新过程。因此，计算量远高于前向传播。
However, in backward propagation, the latency of each layer mainly comes from the partial derivation of the parameters $\sigma_l$ and the calculation of input $x_l$ at each layer and also includes the updating process of the model, as in Eq.~\ref{e2},
\begin{equation} \label{e2}
T_{b} = \sum_{l=1}^L{t_a( \frac{\partial t}{\partial \sigma_l}, x_l) + t_b(\sigma_l)},
\end{equation}
where $t_a(\frac{\partial t}{\partial \sigma_l}, x_l)$ is $l$ the latency of gradient calculation, $t_b(\sigma_l)$ is latency in other procedures of back propagation.
The more complex gradient calculations bring greater computational latency for backward propagation than forward.
%我们观察到，网络在分配计算资源时，时延在每一层的分配也是无差别的。
From Eq.~\ref{e2}, we observe that when performing test-time adaptation, the distribution of latency is undifferentiated at each layer.
However, the importance of each layer is different during model adaptation and the accuracy gain is nearly equivalent to updating the entire model if unimportant layers are frozen.
%因此，一种可能的解决方案是通过停止某一子层的梯度计算来减少向后的计算和延迟。
Therefore, one effective solution to reduce adaptation latency is to reduce backward computation and latency by stopping gradient computation at unimportant DNN model portion.
%已有研究表明，仅更新部分层甚至可以获得比更新整个模型更高的准确率\cite{evci2022head2toe,lee2022surgical}。
Existing research shows that only updating important layer even can get higher accuracy than the entire model as it reduces model overfitting issues during adaptation~\cite{evci2022head2toe, lee2022surgical}. 
%这提供了一个机会，我们可以只更新重要层的准确性，这样就可以在保持自适应精度的同时降低时延。
This provides an opportunity to update the accuracy of only the important layers so that we can reduce latency while maintaining adaptive accuracy.

%然而，后向延迟与冻结层的数量并不完全成正比关系。
However, the backward latency is not completely proportional to the number of freezing layers.
%如图\ref{fig:layernum_latency}所示，更新第一层的向后延迟与更新后四层的延迟相同。
As shown in Figure~\ref{fig:layernum_latency}, the backward latency for updating the first layer is the same as the latency for updating the last four layers.

\begin{figure}[t]
  \centering
  \includegraphics[width=.83\linewidth]{figure/layernum_latency.pdf}
  \caption{Example of Latency in Updating. GC means gradient calculation. Both updating one layer and updating four layers result in the same GC computation latency.}
  \label{fig:layernum_latency}
\end{figure}
%因为在后向阶段，每个层的更新都依赖于当前层的梯度图，因此为了得到当前层的计算结果，我们需要计算先前所有层的梯度。
Because the updating of each layer depends on the gradient of the current layer in the backward stage, we need to calculate the gradient of all previous layers to get the final result of the current layer.
%因此，我们不仅需要考虑优化更新层的数量，同时也需要考虑第一更新层的位置。
Therefore, we need to consider not only the number of optimized updating layers but also the location of each updating layer.

%基于以上的观察，我们选择稀疏更新也为优化后向延迟提供了机会。
% 在完全更新时，模型中的所有层在向后更新后都会发生变化，需要基于完全更新后的模型对所有层进行顺序向后更新。
% 在稀疏更新中，frozen layer的\(w_l\)在适应周期中保持不变。因此，在reforward过程中，这些层可以在forward阶段重用它们的输出，避免冗余计算并减少reforward中的延迟:
% \begin{equation} \label{d4}
%     T_{refor}=g\left( B \right) =\sum_{l=\min B}^L{t_{fw_l}},
% \end{equation}
% 所有层的\(\delta w_l\)和\(\delta x_l\)的计算导致了后向阶段的更高延迟。

% To optimize the latency of test-time adaptation in mobile scenarios, we first analyze the efficiency of test-time adaptation in mobile scenarios. Typically, test-time adaptation is divided into an adaptation and an inference. In adaptation stage, the model updates the weights once based on current input data from mobile scene. Specifically, model adaptation is accomplished by constructing a computational graph through forward and accomplishing the model update through once backward. In inference stage, the adapted model infers again. 
% Therefore, online once-adaptation cycle consists of three stages: forward, backward, and reforward, as Eq.~\ref{d1}
% \begin{equation} \label{d1}
%     T_{ada}=T_{for}+T_{back}+T_{refor}
% \end{equation}
% where $T_{for}$, $T_{back}$ and $T_{refor}$ are the latency of forward, backward, and reforward.
% We analyze the latency of these stages, as shown in Fig.~\ref{fig:forward_backward_latency}.



% We find that the latency of backward is much larger than that of forward during the adaptation cycle in mobile scenarios. 
% Therefore, our main goal is to optimize the latency of backward and further optimize other processes as well. 

% We further explored the reasons behind the higher latency in backward stage.
% In forward stage, model only need to sequentially calculate the forward output of each layer, as Eq.~\ref{d3}:
% \begin{equation} \label{d3}
%     T_{for}=\sum_{l=1}^L{t_{fw_l}},
% \end{equation}
% In backward stage, latency primarily comes from the gradient calculation for each layer's parameters \(w_l\) and input \(x_l\) and more calculation than forward result in higher backward latency:
% \begin{equation} \label{d2}
%     T_{back}=f_{\delta x_l}\left( B \right) +f_{\delta w_l}\left( B \right) =\sum_{l=\min B+1}^L{t_{\delta x_l}}+\sum_{l\in B}{t_{\delta w_l}},
% \end{equation}
% where \(B\) is the set of updating layers, and \(\min B\) is the minimum index of layers in \(B\). DNN model performs a fully update with the maximum backward latency when \(B\) includes all layers.

% Therefore, a potential solution is to reduce calculation and latency of backward by stopping the gradient computation for a subset of layers.

% %For different types and degrees of distributional offsets, different layers show different importance of accuracy in the adaptation process~\cite{evci2022head2toe,lee2022surgical}. 
% Previous researches show that updating only some layers may even result in higher accuracy than that of updating the entire model~\cite{evci2022head2toe,lee2022surgical}. This provides an opportunity to optimize backward latency through only updating important layers to accuracy while maintaining adaptation accuracy.
% However, backward latency is not fully proportional to the number of frozen layer parameters. As shown in Fig.~\ref{fig:layernum_latency}, the backward latency for updating the first layer is the same as the latency for updating the last four layers. Because in backward stage, each layer's updating depends on the layer input's gradient calculation for all subsequent layers.
% Therefore, optimizing both the number of updating layers and the position of the first updating layer is necessary to reduce backward latency.

% Sparse update also brings an opportunity to optimize reforward latency.
% In full update, all layers in the model change after backward, requiring the sequentially reforward of all layers based on the full updated model.
% In sparse update, frozen layer's \(w_l\) remains unchanged during adaptation cycle. As a result, during reforward, these layers can reuse their outputs in forward stage, avoiding redundant computations and reducing the latency in reforward:
% \begin{equation} \label{d4}
%     T_{refor}=g\left( B \right) =\sum_{l=\min B}^L{t_{fw_l}},
% \end{equation}
% The computation of \(\delta w_l\) and \(\delta x_l\) for all layers leads to the higher latency in the backward stage. 









%\noindent \textbf{Layer Latency Difference.}  Therefore, the adaptation latency is not proportional to the number of frozen layer parameters, freezing more parameters does not necessarily reduce more latency.
%因此？？？这里应该有一个公式表达这个观点，想象一个n层的网络，网络反传的时间是一个单调递增函数，如   ？，所以XXX。 As shown in Fig.~\ref{layernum_latency}, one layer's updating latency is the same as four layers' latency.

% The adaptation latency is not proportional to the number of participants involved in adaptation, which is mainly due to the principle of backpropagation. As shown in Fig.~\ref{layernum_latency}, one layer's updating latency is the same as four layers' latency.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.76\linewidth]{figure/layernum_latency.pdf}
%   \caption{Time of sparse update. GC means gradient calculation. Both updating one layer and updating four layers result in the same 8 times GC computation.}
%   \label{fig:layernum_latency}
% \end{figure}


%为了在移动场景下优化TTA算法的时延，我们首先对TTA算法在移动场景下的时效进行了分析。
%通常来讲，TTA主要可以分为两个阶段：适应阶段和重推理阶段。
%在适应阶段，模型将依赖当前移动场景的信息进行权重更新。
%具体来说，推理数据通过正向传播过程构建计算图，依靠反向传播完成模型更新，这样完成单次模型适应。
%而在推理阶段，通过适应后的模型，完成对输入数据的推理。
%我们对这两个过程的一般时延进行了分析，如图所示。
%图
%我们观察到，在移动场景下的自适应阶段，反向传播过程的时延远大于正向传播的时延。因此我们的首要目的是优化反向传播带来的时延，此外进一步优化其他过程。在此过程中有如下挑战：

%时延差异。因此适应时延和参与适应的参数量并非正比关系，这主要由于反向传播的原理决定，
%重要性差异。对于不同类型和程度的分布偏移，不同的层在适应中过程显示出了不同的精度重要性~\cite{}，只适应最重要的一部分层的精度甚至提升比微调整个模型的精度提升更高。这给在保持适应精度的情况下用模型稀疏更新来加速适应过程带来了时延优化机会。


%模型在云端预训练完成对通用场景数据的学习，在移动设备上只需要针对模型部分层执行适应性微调而非从头训练以适应新场景数据的分布偏移。
%对于不同类型和程度的分布偏移，不同的层在适应中过程显示出了不同的精度重要性~\cite{}，只适应最重要的一部分层的精度甚至提升比微调整个模型的精度提升更高。这给在保持适应精度的情况下用模型稀疏更新来加速适应过程带来了时延优化机会。
%为了优化时延，我们对适应时延的bottleneck--反向传播进行稀疏化。然而在移动环境下实时数据流和cloud pre-train数据间的distribution shift的类型和程度是潜在和难以刻画的。关键挑战是如何在当前未知分布的实时数据下，快速评估NN模型每层的微调重要性，并在满足时延优化目标的约束下选取最重要的层执行稀疏反向传播和更新。

%第二阶段，重新对当前数据进行推理，得到最终的推理结果。由于模型面向当前数据进行了优化，使得更适合于

% forward计算中间激活，逐步跟踪和建立backward计算图，
% backward基于中间激活和计算图执行梯度计算和参数更新过程，完成模型适应，
% reforward基于适应后的模型完成对输入数据的推理
%先前的


%方法级别的论述


%因此，我们使用XX方法来提高对层重要性的实时评估(见A节)，动态监测各层的运行时延迟并进行在线搜索(见B节)。在撰写论文时，我们应该使用简洁清晰的语言，以确保读者能够轻松理解我们的研究内容。


% Although sparse updates can help accelerate test-time adaptation, how to build sparse updates for mobile scenarios remains a challenge. 
% Previous sparse update methods mainly aimed to optimize training speed (reference), but in mobile scenarios, they face the following challenges:

% \noindent \textbf{Importance of Layers} Sparse updates need to adapt to the real-time changes of data online, which requires frequent evaluation of layer importance. Previous methods mainly used strategy A or B for this process, as shown in the table (reference), but this does not meet the requirement of real-time performance.

% \noindent \textbf{Online} Previous sparse update strategies usually use offline evaluation, but the delay of mobile devices can change during actual execution, which requires online evaluation of the delay of each process. Therefore, offline searching will lead to inaccurate search results.

% Therefore, we use XX method to improve the real-time evaluation of layer importance (see Section A), dynamically monitor the runtime delay of each layer and conduct the online search (see Section B). When writing the paper, we should use concise and clear language to ensure that readers can easily understand our research content.

% 尽管稀疏更新可以帮助TTA加速，但在移动场景下，如何为移动场景构建稀疏更新依然是是一种挑战。
% 之前的稀疏更新主要目标是优化训练速度~\cite{}，但是，其在移动场景下存在以下挑战：

% 层重要性评估。
% 在移动场景下，稀疏更新需要在线适应数据的实时变化，这导致了需要频繁评估层重要性。之前的方法主要通过A或者B策略进行这个过程，如表所示~\ref{}，这不满足实时性的要求。

% 离线 vs 在线。
% 之前的稀疏更新策略通常采用离线评估，但移动设备在实际执行时延会变化，这需要在线评估各个流程的时延。因此，离线搜索会导致搜索结果不准确。

% 因此，我们通过XX，提高了层重要性评估的实时性 in Sec A，同时，我们的评估动态的监控每层的运行时延，进行在线搜索 in Sec B。


% 对第一个，简单说就是基于每层在当前输入分布下，该层输出数据的一阶和二阶统计，和历史场景的统计间的KL距离来表示该层参数在当前分布偏移下的泛化能力，代表着这一层更新的必要性，距离越大代表着这一层参数不能handle当前场景，需要更新来让参数适应新场景，重要性高。

% 对第二个，首先分析每层的执行时延来源于计算时延+访存时延，然后分别分析这两个时延会受到哪些动态硬件资源影响而改变。然后建模，在某种硬件资源条件下，基于每层的离线时延预测当前实际执行时延

% 目前的 test-time adaptation 方法对归一化层或所有层采用统一的更新方法，导致模型更新过程中的计算冗余和复杂性增加，这对移动场景下的模型效率产生了负面影响。稀疏更新（Sparse updating）作为一种模型更新加速技术被引入~//cite{}。通过剪枝计算图，稀疏更新可以在一定程度上减少后向过程的延迟。然而，这种方法仍然需要针对移动环境中的动态硬件环境和数据分布进行优化。

% \noindent \textbf{Dynamic device resources.} 延迟是一个动态指标，在同一设备上执行相同操作的延迟可能会因设备条件而变化~\cite{}。以往的稀疏更新方法依赖于离线测量的延迟信息，用于重新训练时的策略搜索~/cite{}。由于重新训练很少与其他计算任务同时进行，因此离线测量与重新训练环境之间的延迟差异很小。然而，在测试阶段，该方法与设备上的其他进程同时运行，必须争夺设备资源，而且硬件条件可能会发生重大变化。现有的延迟分析方法主要预测理想黑盒设备条件下的执行延迟，忽略了动态设备条件对延迟的影响。为了达到预期的加速效果，有必要对当前设备条件下各层的精确延迟进行实时分析。

% \noindent \textbf{Dynamic data distribution.} 稀疏更新需要精确的层重要性，以确保获得的更新策略能达到预期的精度提升。在模型训练过程中，各层的重要性并不是固定不变的，而是根据新场景数据集和云数据集之间的分布偏移而变化~\cite{}。在 test-time adaptation 环境中，实时数据流的分布是未知且不断变化的，因此需要频繁评估每批数据的层重要性。以往的稀疏更新策略需要在相同分布的微调数据集上进行训练，只需要偶尔评估层重要性。然而，这些评估的延迟成本很高，有时甚至超过了训练本身，因此在实时数据流场景中需要频繁评估时，会造成巨大的开销和模型效率的降低。

% The time efficiency of test-time adaptation is impacted by the notable differences in latency and importance among various layers in neural networks. Current test-time adaptation methods apply a uniform updating approach to normalization layers or all layers~\cite{}, leading to computational redundancy and increased complexity during model updates~\cite{}, which negatively affects the model efficiency in mobile scenarios. Sparse updating has been introduced as an acceleration technique for model updates~\cite{}. By pruning the computational graph, sparse updating can reduce the latency of the backward process to some extent. However, this method still requires optimization for dynamic hardware environments and data distributions in mobile settings.

% \noindent \textbf{Dynamic device resources.} Latency is a dynamic metric, and the latency of performing the same operation on the same device may vary due to device conditions~\cite{}. Previous sparse updating methods rely on offline-measured latency information for policy search during retraining~\cite{}. Since retraining rarely occurs alongside other computational tasks, the latency difference between offline measurements and retraining environments is minimal. However, during the testing phase, which runs concurrently with other processes on the device, the method must compete for device resources, and hardware conditions may change significantly. Existing latency analysis methods mainly predict the execution latency under ideal black-box device conditions, ignoring the impact of dynamic device conditions on latency. To achieve the expected acceleration effect, real-time analysis of the precise latency for each layer under current device conditions is necessary.

% \noindent \textbf{Dynamic data distribution.} Sparse updating requires accurate layer importance to ensure the expected accuracy improvement in the obtained update policies. The importance of each layer during model training is not fixed but varies based on the distribution offset between the new scene dataset and the cloud dataset~\cite{}. In a test-time adaptation environment, the distribution of real-time data streams is unknown and constantly changing, necessitating frequent evaluation of layer importance for each data batch. Previous sparse updating strategies involve training on identically distributed fine-tuned datasets and only require occasional evaluations of layer importance. However, these evaluations have high latency costs, sometimes exceeding the training itself, resulting in significant overhead and reduced model efficiency when frequent evaluations are needed in real-time data streaming scenarios.

% % \subsection{Sparse Updating on Moblie Device}
% The time efficiency of test-time adaptation is impacted by the notable differences in latency and importance among various layers in neural networks. Current test-time adaptation methods apply a uniform updating approach to normalization layers or all layers~\cite{}, leading to computational redundancy and increased complexity during model updates~\cite{}, which negatively affects the model efficiency in mobile scenarios. Sparse updating has been introduced as an acceleration technique for model updates~\cite{}. By pruning the computational graph, sparse updating can reduce the latency of the backward process to some extent. However, this method still requires optimization for dynamic hardware environments and data distributions in mobile settings.

% \noindent \textbf{Dynamic device resources.} Latency is a dynamic metric, and the latency of performing the same operation on the same device may vary due to device conditions~\cite{}. Previous sparse updating methods rely on offline-measured latency information for policy search during retraining~\cite{}. Since retraining rarely occurs alongside other computational tasks, the latency difference between offline measurements and retraining environments is minimal. However, during the testing phase, which runs concurrently with other processes on the device, the method must compete for device resources, and hardware conditions may change significantly. Existing latency analysis methods mainly predict the execution latency under ideal black-box device conditions, ignoring the impact of dynamic device conditions on latency. To achieve the expected acceleration effect, real-time analysis of the precise latency for each layer under current device conditions is necessary.

% \noindent \textbf{Dynamic data distribution.} Sparse updating requires accurate layer importance to ensure the expected accuracy improvement in the obtained update policies. The importance of each layer during model training is not fixed but varies based on the distribution offset between the new scene dataset and the cloud dataset~\cite{}. In a test-time adaptation environment, the distribution of real-time data streams is unknown and constantly changing, necessitating frequent evaluation of layer importance for each data batch. Previous sparse updating strategies involve training on identically distributed fine-tuned datasets and only require occasional evaluations of layer importance. However, these evaluations have high latency costs, sometimes exceeding the training itself, resulting in significant overhead and reduced model efficiency when frequent evaluations are needed in real-time data streaming scenarios.

%由于神经网络中不同层所导致的时延和重要性存在显著的差异，这影响了TTA的时间效率。
%但是，由于当前的TTA~\cite{}对于神经网络各层均采用了无差异化的更新模式，在模型更新过程中会造成计算冗余和复杂度提高，从而影响移动场景下的模型效率。
%为了解决这个问题，稀疏更新~\cite{}近年来被提出作为一种加速模型更新的手段。
% ！！！补充：稀疏更新的原理（直截了当）稀疏更新是XXX，为了XXX，XXX
%稀疏更新通过对计算图进行剪枝，从而一定程度上减少反向传播过程的时延。
%但是，这种方法依然需要针对移动场景动态的硬件环境和数据分布进行优化。
% \noindent \textbf{Dynamic device resources.} 时延是一个动态性指标，即使在同一个设备上执行同一个操作的时延也会随着设备条件的变化而变化。先前的稀疏更新方法基于离线环境测量的每层时延信息完成重训练时的策略搜索。因为重训练很少与其他计算任务共同执行,因此离线测量环境和重训练环境（通常在深夜）下的时延相差很小\cite{}。然而测试时适应在设备推理时运行（例如白天），这意味着它需要和设备上更多的其他进程同时竞争设备资源，例如无人机的控制程序、手机的应用程序。并且设备的硬件条件如温度也可能发生大幅变化。现有的时延分析方法\cite{}主要预测给定网络结构在黑盒设备理想条件下的执行时延。忽略了运行时动态的设备条件给时延带来的影响。为了让策略实际加速效果符合预期，需要实时分析当前设备条件下每一层准确的时延。

% \noindent \textbf{Dynamic data distribution.} 稀疏更新方法需要准确的层精度重要性以保证搜索得到的更新策略能实现预期精度提升。模型训练时每层的精度重要性不固定，而是根据新场景数据集与云端数据集间分布的偏移类型和程度而改变[surgical,和它的引文]。TTA环境下实时数据流的分布未知并且实时变化，因此需要对每一批次的数据频繁评估其对应的层精度重要性。先前的稀疏更新策略[ET,256KB]在同分布的微调数据集上完成训练，因此只需要在多轮训练中一次性（离线单层微调[256KB]方法）或定期（基于完整反向传播[ET]的梯度方法）评估层精度重要性。但这些评估的时延成本较高甚至超过训练本身，因此在需要频繁评估的实时数据流条件下，会造成极高的开销，严重影响模型的效率。

%%%%%方程原文：
%稀疏更新具有提升TTA时间效率的潜力，但是，这种方法依然需要针对移动场景动态的硬件环境和数据分布进行优化。
% \noindent \textbf{Dynamic device resources.} 时延是一个动态性指标，即使在同一个设备上执行同一个操作的时延也会随着设备条件的变化而变化。先前的稀疏更新方法基于离线环境测量的每层时延信息完成重训练时的策略搜索。因为重训练很少与其他计算任务共同执行,因此离线测量环境和重训练环境（通常在深夜）下的时延相差很小\cite{}。然而测试时适应在设备推理时运行（例如白天），这意味着它需要和设备上更多的其他进程同时竞争设备资源，例如无人机的控制程序、手机的应用程序。并且设备的硬件条件如温度也可能发生大幅变化。现有的时延分析方法\cite{}主要预测给定网络结构在黑盒设备理想条件下的执行时延。忽略了运行时动态的设备条件给时延带来的影响。为了让策略实际加速效果符合预期，需要实时分析当前设备条件下每一层准确的时延。

% \noindent \textbf{Dynamic data distribution.} 稀疏更新方法需要准确的层精度重要性以保证搜索得到的更新策略能实现预期精度提升。模型训练时每层的精度重要性不固定，而是根据新场景数据集与云端数据集间分布的偏移类型和程度而改变[surgical,和它的引文]。TTA环境下实时数据流的分布未知并且实时变化，因此需要对每一批次的数据频繁评估其对应的层精度重要性。先前的稀疏更新策略[ET,256KB]在同分布的微调数据集上完成训练，因此只需要在多轮训练中一次性（离线单层微调[256KB]方法）或定期（基于完整反向传播[ET]的梯度方法）评估层精度重要性。但这些评估的时延成本较高甚至超过训练本身，因此在需要频繁评估的实时数据流条件下，会造成极高的开销，严重影响模型的效率。











%云端训练数据往往无法涵盖所有的移动场景，导致模型在移动端部署后还需要重训练（适应）来维持预测精度。
%目前移动端的微调模式是离线重训练：预先收集并标注目标部署场景的数据样本，随后进行持续数十个小时的设备端训练【cite melon，et，sage】。
%然而，标注数据和训练过程非常耗时，这意味着重训练过程只能离线进行，新场景中的推理任务必须等重训练过程结束后才能开始。
%当移动设备面临的场景频繁切换时，需要不断执行数据标注和重训练过程。
%此外，在模型部署和推理前就收集到新场景的训练数据可能十分困难甚至不可能，例如在无人机监测任务中，提前一天收集无人机第二天将要部署环境的数据。
% Cloud data for training fails to cover all mobile scenarios, resulting in the adaptation of DNN model on mobile devices to maintain inference accuracy after deployment. 
% The common adaptation mode on mobile devices is offline retraining: pre-collecting and annotating samples from deployment scenarios, followed by offline multi-epoch training on device\cite{} or cloud\cite{}.
% However, data annotation and offline retraining are time-consuming\cite{}. So inference tasks in new scenarios must wait to begin until the offline retraining is completed.
% When mobile devices frequently encounter different scenes, it has to continually perform data annotation and offline retraining which significantly affects the efficiency of mobile task execution.
% In addition, collecting retraining data in new scenarios before DNN model deployment is challenging. For example, in tasks such as drone surveillance\cite{} and autonomous driving\cite{}, pre-collecting data in environment where the device will be deployed the next day is impossible.


%测试时适应（test-time adaptation），又称为无源域适应（source-free domain adaptation），是域适应领域的一种无监督训练模式。
%TTA的模式十分适用于连续变化的移动端场景：不需要预先进行任何数据准备和离线训练，仅在真正执行推理任务时基于当前需要推理的数据完成无监督的模型适应。
%TTA主要包括三个阶段：forward-backward-reforward。
%在forward和backward阶段，模型基于当前数据完成一轮反向传播。
%在reforward阶段，完成适应的模型再次对当前数据完成推理。
%这三个阶段是在模型推理时在线运行的，因此backward和reforward的执行时延直接影响了模型推理移动端数据流的帧率。

%然而将现有的TTA方法部署在移动设备上时，移动设备有限的算力会产生较高的计算时延，这严重影响了模型推理数据流的效率。

%此外，测试时适应和离线训练并不冲突，可以耦合使用以进一步提高推理精度：在部署前基于新场景数据集完成通用性离线适应，在执行推理任务时对当前输入样本进行针对性在线适应。
% Test-Time Adaptation(test-time adaptation)\cite{} is an unsupervised adaptation mode in the field of domain adaptation\cite{}. 
% It's worth noting that test-time adaptation and offline retraining can be coupled for further improving inference accuracy. 
% Generic offline adaptation based on new scenario dataset can be completed before deployment, and targeted online adaptation can be performed on inference data input during tasks execution.
% test-time adaptation is suitable for dynamic mobile scenarios because test-time adaptation don't need data annotation and offline retraining. 
% Instead, model adaptation is performed online only based on unsupervised inference data stream when tasks execute.
% test-time adaptation involves three stages\cite{liang2023comprehensive}: forward, backward, and reforward.
% During forward and backward, model completes adaptation with once forward propagation and backward propagation based on inference data input. 
% In reforward, adapted model performs inference again on inference data input.
% Three stages online execute during inference, so the latency of backward and reforward directly affects the inference efficiency on mobile data stream.
% However, as shown in Figure 2-1, deploying existing test-time adaptation methods on mobile devices will results in high latency which impacts efficiency of inference due to limited computational capability.


% \subsection{Opportunities for test-time adaptation Speedup}
%现有的TTA方法致力于解决在连续适应条件下错误累计带来的精度下降问题，部署在资源有限的移动端后可能产生性能问题。
%我们首先分析这些方法在移动端设备上的适用性。
%一类方法通过减小伪标签对整个模型参数的影响来减轻错误累计问题，这些方法只更新模型的BN层或其他标准化层的参数。
%但由于反向传播计算具有依赖性，因此适应时延和参与适应的参数量并非正比关系。
%如图xx（a）所示，尽管只更新第一层参数，但需要反向计算整个网络的梯度，适应时间和更新后四层的四倍参数的时间相同。因此尽管这些方法只更新小部分参数，但依然会导致非常高的适应时延。因为反向传播计算具有依赖性，适应时延和参与适应的参数量并非正比关系。并且只更新少量的标准层参数会影响模型的适应能力，导致适应后精度提升有限~\cite{cotta}。
%另一类方法在适应时通过提高伪标签的可信度来减轻错误累计问题，更可靠的伪标签让这些方法即使更新整个模型的参数也能够保持连续适应后的精度。然而，计算更准确的伪标签会带来额外的计算成本（例如cotta的多个伪标签融合~\cite{cotta}），并且更新整个模型需要完整的反向传播计算。这会导致当这些方法部署在移动设备上时会产生较高的在线适应时延，从而影响模型的推理效率。
%相比于从头训练，模型在移动端部署后的适应是为了微调参数以适应新场景数据和云端训练数据间的分布差异。
%对于不同类型和程度的分布偏移，不同的层在微调中过程显示出了不同的重要性~\cite{}，只微调最重要的一部分层的精度甚至提升比微调整个模型的精度提升更高。这给在保持微调精度的情况下用模型稀疏更新来加速微调过程带来了时延优化机会。然而在缺乏数据集类型等元信息的真实场景中，实时数据的分布偏移类型和程度是潜在和难以刻画的。因此关键挑战是如何对移动场景t时刻的数据流，实现模型每层对应微调重要性的建模。
%如果进一步考虑更新每层给模型适应带来的时延开销，并权衡精度-时延进行搜索，就能够在实现低时延的同时保持模型适应带来的精度收益。此外，只更新部分参数还能够减轻连续适应带来的错误累计现象。
% Existing test-time adaptation methods aim to solve accuracy decline caused by error accumulation after continuous unsupervised adaptation. 
% So when deployed on resource-constrained mobile devices, they may lead to performance challenges. 
% We first analyze the applicability of these methods on mobile devices.


% One kind of test-time adaptation methods solve error accumulation by reducing the impact of wrong pseudo-labels on model parameters. 
% These methods only update parameters of batch normalization(BN) layers\cite{} or other normalization layers\cite{}. 
% However, due to the dependency of backpropagation chain, adaptation latency and the number of updating parameters are not directly related. 
% As shown in Figure xx (a), even only the first layer parameters are updated, the gradients of entire network still need to be computed, resulting in adaptation latency equal to updating last four layers parameters, even latter involves four times more parameters.
% %因此尽管这些方法只更新小部分参数，但依然会导致非常高的适应时延。因为反向传播计算具有依赖性，适应时延和参与适应的参数量并非正比关系。并且只更新少量的标准层参数会影响模型的适应能力，导致适应后精度提升有限~\cite{cotta}。


% Another kind of test-time adaptation methods addresses error accumulation by enhancing confidence of pseudo-labels~\cite{}. 
% More reliable pseudo-labels can maintain accuracy after continuous unsupervised adaptation even updating the parameters of the entire model. 
% %然而，计算更准确的伪标签会带来额外的计算成本（例如cotta的多个伪标签融合~\cite{cotta}），并且更新整个模型需要完整的反向传播计算。这会导致当这些方法部署在移动设备上时会产生较高的在线适应时延，从而影响模型的推理效率。

% %相比于从头训练，模型在移动端部署后的适应是为了微调参数以适应新场景数据和云端训练数据间的分布差异。对于不同类型和程度的分布偏移，不同的层在微调中过程显示出了不同的重要性~\cite{}，只微调最重要的一部分层的精度甚至提升比微调整个模型的精度提升更高。这给在保持微调精度的情况下用模型稀疏更新来加速微调过程带来了时延优化机会。然而在缺乏数据集类型等元信息的真实场景中，实时数据的分布偏移类型和程度是潜在和难以刻画的。因此关键挑战是如何对移动场景t时刻的数据流，实现模型每层对应微调重要性的建模。
% %如果进一步考虑更新每层给模型适应带来的时延开销，并权衡精度-时延进行搜索，就能够在实现低时延的同时保持模型适应带来的精度收益。此外，只更新部分参数还能够减轻连续适应带来的错误累计现象。



% \subsection{Sparse Updating in Online Adaptation}
%测试时适应在模型推理时在线运行，复杂且动态的移动端环境、给适应过程带来了两个挑战：动态的硬件环境和数据分布。
% test-time adaptation runs online during device executes tasks. Compared to offline training conditions, complex and dynamic runtime conditions bring two challenges to online adaptation: dynamic device resources and data distributions.

% \textbf{Dynamic device resources.}
% \label{Dynamic device resources.}
%稀疏更新方法需要准确的层时延信息以保证搜索得到的更新策略符合预期加速效果。和内存、能耗等指标不同，时延是一个动态性指标，即使在同一个设备上执行同一个操作的时延也会随着设备条件的变化而变化。先前的稀疏更新方法基于离线环境测量的每层时延信息完成重训练时的策略搜索。因为重训练很少与其他计算任务共同执行,因此离线测量环境和重训练环境（通常在深夜）下的时延相差很小\cite{}。然而测试时适应在设备推理时运行（例如白天），这意味着它需要和设备上更多的其他进程同时竞争设备资源，例如无人机的控制程序、手机的应用程序。并且设备的硬件条件如温度也可能发生大幅变化。现有的时延分析方法\cite{}主要预测给定网络结构在黑盒设备理想条件下的执行时延。忽略了运行时动态的设备条件给时延带来的影响。为了让策略实际加速效果符合预期，需要实时分析当前设备条件下每一层准确的时延。
% Sparse update requires accurate layer latency estimate to ensure that update strategy can achieve expected acceleration goal.
% Latency is a highly dynamic metric and even the latency of the same operation executed on the same device varies with different device resources.
% Previous sparse update methods search update strategy based on offline once estimate of layer latency\cite{} and strategy works well during retraining.
% Because offline retraining is rarely performed concurrently with other computational tasks(typically executed during night), hardware resources between estimate and retraining are minimal\cite{huang2023elastictrainer}.
% However, test-time adaptation runs during device executes tasks(typically during the day), which means it needs to share device resources with more other computational processes on device, such as flight control program of a drone or applications of a smartphone. 
% Additionally, device hardware conditions such as temperature, may significant changes.
% These factors result in significant discrepancies between actual execution latency and offline estimate latency of the same layer.
% Existing latency analysis methods\cite{} primarily predict execution latency of a given network structure under offline conditions of a black-box device. 
% However, these methods ignore the impact of dynamically changing device conditions on latency during runtime. 
% To ensure that actual acceleration goal align with searched strategy expectations, it is necessary to predict actual execution latency of each layer under dynamic device conditions.




% \textbf{Dynamic data distribution.}
% \label{Dynamic data distribution.}
%稀疏更新方法需要准确的层精度重要性以保证搜索得到的更新策略能实现预期精度提升。模型训练时每层的精度重要性不固定，而是根据新场景数据集与云端数据集间分布的偏移类型和程度而改变[surgical,和它的引文]。TTA环境下实时数据流的分布未知并且实时变化，因此需要对每一批次的数据频繁评估其对应的层精度重要性。先前的稀疏更新策略[ET,256KB]在同分布的微调数据集上完成训练，因此只需要在多轮训练中一次性（离线单层微调[256KB]方法）或定期（基于完整反向传播[ET]的梯度方法）评估层精度重要性。但这些评估的时延成本较高甚至超过训练本身，因此在需要频繁评估的实时数据流条件下，会造成极高的开销，严重影响模型的效率。
% Sparse update requires accurate layer accuracy importance to ensure that update strategy can achieve expected adaptation accuracy improvement.
% Accuracy importance of each layer during training is not fixed but rather changes based on the type and level of distribution shift between mobile scene data and cloud data\cite{surgical, and its references}.
% The distribution of online data stream in test-time adaptation is unknown and continuously changing. 
% Therefore, it is necessary to frequently estimate layer accuracy importance for online data stream.
% Previous sparse update methods\cite{huang2023elastictrainer, lin2022device} focus on offline retraining on independent and identically distributed(IID) fine-tuning dataset. 
% Therefore, these methods only execute layer accuracy importance estimation either once (offline single-layer fine-tuning\cite{lin2022device}) or periodically (gradient-based method through complete backward\cite{huang2023elastictrainer}) during multiple training epochs.
% However, once execution latency of these evaluation methods is equal to or even exceeds once backward during training, as shown in Figure xx. 
% Therefore, frequent evaluations will lead to extremely high latency on online data stream, severely impacting the efficiency of DNN model.





%\subsection{Sparse updating for Responsive Adaptation}
%在TTA中，对于一批输入数据，模型需要先完成在线适应后才能给出预测结果。因此模型适应的速度十分重要，直接决定了模型预测的速度，特别是在无人机监测等对时延要求较高的场景中。然而，目前的TTA方法聚焦于提高无监督训练的可信度和训练精度，并面向服务器设备展开设计和验证。当这些TTA方法部署在资源有限的移动端设备时，会造成较高的适应时延，严重影响了设备端任务预测的速度。最近，XX等人提出了第一个内存高效的on-device TTA方法——EcoTTA，which通过避免存储主干网络的中间激活来减少内存消耗。然而，EcoTTA在部署时依然会面临高时延的挑战，如图xx所示\cite{}。
%稀疏更新技术通过稀疏化模型训练时延的bottleneck——反向传播计算，来加快模型训练的速度或减少训练内存占用。在调研了设备端训练加速技术后，我们发现稀疏更新是加速测试时适应的理想技术。第一，在无监督训练中，伪标签带来的可能性错误监督会导致模型在多轮适应后的精度不断下降甚至崩塌，叫做错误累计现象。为了应对错误累计，TTA方法通常只更新模型的一部分参数，例如BN层【cite：tent，eata】，来减轻累计错误对模型的影响。因此稀疏更新有机会同时解决适应时延问题和错误累计问题。第二，稀疏更新能够通过控制反向传播的稀疏程度实现对适应速度快慢的动态调整，这在预测数据流等对帧率有灵活要求的任务中尤其重要。其他技术例如计算卸载技术在缺少DSP等结构的设备上难以适用，量化技术带来的精度损失会在无监督适应中进一步放大。但如果需要进一步加速，稀疏更新技术作为一种更新模式，能够方便地和这些技术耦合使用。


==> body/others/design.tex <==


\subsection{Overview}
In this section, we will first give an overview of SwiftTTA, then elaborate its each work stage.

\textbf{Design goal}
%设计目标：SwiftTTA的目标是在给定数据流预测帧率需求的情况下最大化模型的测试时适应精度。在移动部署环境中，帧率需求通常由算法开发人员固定，或根据场景切换而在运行时动态调整。
\textbf{Design Objective:}The goal of SwiftTTA is to maximize the test-time adaptation accuracy of the model while meeting the specified frame rate requirements for a given data stream. In mobile deployment environments, frame rate requirements are typically fixed by algorithm developers or dynamically adjusted at runtime based on scene changes.
%SwiftTTA基于稀疏更新方法，通过调整参与模型适应的层集合来调整模型适应过程中时延的bottleneck部分——BP，并同时利用tensor save-load机制调整第二次前向传播的时延，从而实现对数据流预测帧率的灵活控制。这一问题被表述为如下约束优化问题：
%%%%%公式0
%其中xx是xx。
%为了在满足预测帧率的条件下最大化模型适应的精度收益，需要选择最重要的层集合参与更新，因此需要评估每层如果参与更新，预期带来的精度收益和时延成本。然而相比离线训练，模型在预测实时数据流时适应会产生数据偏移和硬件状态实时发生未知变化的问题，因此SwiftTTA的关键设计包括两个具有实时性的layer profiler——layer accuracy benefit profiler（4.3节）和layer latency overhead profiler（4.4节）。此外，SwiftTTA还通过tensor saver-loader机制进一步减少了未参与更新更新层带来的冗余Reforward时延，如4.5节所示。

\textbf{Workflow}
%Workflow。如图xx所示，SwiftTTA分三个阶段完成模型的适应和预测。在Forward stage，SwiftTTA执行首次前向传播并更新层信息；在Backward stage，SwiftTTA搜索最优层更新集合，并基于第一阶段执行反向传播计算；Reforward stage，
\begin{itemize}
    \item \textbf{Forward stage}. 
    %（1）在Forward stage，SwiftTTA对当前批次数据执行前向传播计算并实时完成对模型每层精度和时延信息的更新。首先，layer accuracy benefit profiler基于层间激活实时生成当前批次数据的分布统计信息并计算和历史数据分布间的KL-divergence；layer latency overhead profiler基于当前硬件状态（包括计算设备温度、系统竞争进程数和缓存命中率）和理想环境下每层的静态时延更新layer latency overhead。   \item \textbf{Backward stage}. 
    %（2）在Backward stage，SwiftTTA搜索需要更新的层并完成对模型的部分反向传播计算。首先基于forward stage更新的层信息执行搜索，得到针对当前批次数据的层更新策略。随后在计算图中保留第一个更新层的激活后，根据层更新策略执行部分反向传播计算图，完成适应。
    \item \textbf{Reforward stage}. 
    %（3）在Reforward stage，SwiftTTA读取保存的激活，并对适应后的模型重新执行部分前向传播过程，完成预测。
\end{itemize}

\subsection{Layer online-accuracy benefit profiling}
%如\ref{Dynamic data distribution.}所述，每层的训练精度收益在不同的输入数据分布下会发生改变。在测试时适应时，实时数据流的分布未知并且实时变化，因此需要频繁对实时数据流进行层精度收益的快速评估，而现有的稀疏更新方法评估层精度收益的方式时延成本太高。为了设计一种实时的精度收益评估方法，我们重新审视了数据分布偏移和每层的训练必要性之间的关联。实际上，在TTA场景下导致模型预测精度下降的根本原因是新场景的数据分布和预训练集的数据分布差异过大，超出了模型当前的预测范围（即泛化能力），而通过更新模型参数能够使其可预测范围扩展到新的数据分布。例如在域适应中，通过减小源域和目标域数据的分布距离来使模型逐渐适应目标域分布。因此我们从对齐历史数据分布和当前数据分布的角度出发，设计了一种面向数据流实时预测场景的层精度收益评估方法和对应的损失函数，通过计算每层历史激活和当前激活间的分布距离来评估每一层的泛化性，即精度收益。在新的输入分布下，如果某层的当前激活分布和历史激活分布越接近，说明该层越能够将当前未知分布映射到已知分布，即泛化性越强。模型每层的泛化能力不同，在某种输入分布下，泛化性强的层应当较小更新以避免错误累计和过拟合，而泛化性弱的层应当大幅更新以充分适应新数据分布。
%给定一个深度网络 f (x; θ)，其中 x 是输入图像，θ 是参数向量。$H$是模型已经适应的历史分布，$C_t$是当前输入数据的分布。为了保证评估方法的通用性和便捷性，我们不对网络架构或云端训练过程作出任何假设。为了减小提取数据分布的成本，我们仅限于用统计数据来表征分布。现有方法通常通过提取样本高阶矩来获取统计信息[HoMM: Higherorder Moment Matching for Unsupervised Domain Adaptation,Central Moment Discrepancy (CMD) for Domain-Invariant Representation Learning.]，然而在移动环境下我们的数据批次可能较小，因此高阶矩难以提取到准确的数据分布。为了平衡统计信息的准确性和计算成本，并使SwiftTTA能够实现小批量在线适应，我们分别对激活的每个通道进行建模，并提取channel-wise的means and variances：
%%%%%公式1
and variances:
%%%%%公式2
%通过计算fl(x)每个通道的均值和方差并将它们连接，我们得到第l层激活的分布表征D_l_t：
%%%%%公式3
%分布表征D_l_t是由fl(x)逐通道的μlk(fl(x))和σ2lk(fl(x))值组成的K维向量。如图xx所示，以图像数据为例，分布表征能够有效表征当前图像的风格与物体。在网络的浅层，分布表征偏向于表示数据的风格和环境信息；在网络的深层，分布表征偏向于表示数据的语义信息。我们计算第l层当前激活的分布表征D_l_t和历史激活的分布表征D_l_h间的KL-divergence来表示第l层的精度收益Bl:
%%%%%公式4
%该指标反映了对于第l层，当前数据的分布偏离模型可预测范围的程度，即更新第l层的必要程度。由于模型需要不断适应新的场景，因此代表模型已经适应的历史分布$H$也需要随着模型的适应而不断更新。我们利用an exponential moving average technique来跟踪用于模型适应的所有数据的平均分布表征。具体来说，给定当前批次数据的分布表征D_l_t，渐进更新分布表征：
%%%%%公式5
%其中xx ∈ [0, 1]。
%为了在缺少数据标签的情况下训练模型，现有测试时适应方法通常最小化模型最后一层输出的熵来增强模型的置信度。但这种方法忽略了数据本身包含的分布信息，为了充分利用小批次数据，并使层精度收益能够更准确的反映层的更新必要性，我们以减小模型每层的当前激活和历史激活之间的分布表征距离作为优化目标，并设计损失函数：
%%%%%公式6
%由于逐通道提取一阶统计量和二阶统计量的特点，基于分布偏移程度的层精度收益评估方法的是计算友好的。对于vgg16，resnet50和mobilenetv2而言，评估batchsize为16的数据的层精度收益的计算开销分别约为推理的xx%，xx%和xx%。如果将评估过程和推理并行计算则能够进一步减小评估带来的额外开销。评估方法也是存储友好的，储存在设备中的历史数据的分布表征与层数和通道数相关。对于resnet50而言，$H$的大小通常在xxKB左右。


\subsection{Layer online-latency overhead profiling}
%如\ref{Dynamic hardware condition.}所述，每层的实际运行时延在不同的硬件条件下会发生改变。测试时适应通常在设备完成预测任务时在线进行，此时分配给每个应用程序的硬件资源是高度动态的。这意味着SwiftTTA需要和忙碌设备上更多的其他进程同时竞争设备资源，例如无人机的控制程序、手机的应用程序，这给每层的实际执行时延带来了更多的不确定性。为了准确评估动态硬件条件下的层时延，需要首先分析影响层时延的各个组成部分的硬件条件因素。在深度模型的推理和训练过程中，每一层在设备理想环境下的总时延主要由计算时延和访存时延组成：%%%%%公式7。当设备实际运行时，每一层的计算时延和访存时延受当前的主频和cache-hit-rate等不同因素影响而变化。因此第l层的在线运行时延tl在运行环境下与理想环境下的离线时延xx关系可建模为：%%%%%公式8。其中pi1，pi2分别为计算时延和访存时延在实际运行条件下的相比于理想环境下的时延的增加倍数，我们称之为计算膨胀系数和访存膨胀系数。
%每层的计算时延主要受该层的浮点运算次数和设备单位时间内能够执行浮点运算次数的影响。对于相同层和相同设备而言，影响单位时间内能够执行该层的浮点运算次数的因素主要包含竞争进程数和硬件温度（例如CPU、GPU）。%\textbf{竞争进程数}：资源受限的移动设备通常依赖CPU或GPU完成计算。以CPU为例，设备操作系统内核（如Linux）默认采用Round Robin scheduling（RR）公平调度计算进程。导致当竞争进程数上升时，当前计算进程的等待时间也会随之上升。%\textbf{硬件温度}：当设备CPU温度升高时，动态电压频率缩放（DVFS）会通过降低主频控制功耗。这会导致当前计算进程的计算时间上升。
%因此，竞争进程数为n，CPU温度为temon时，计算膨胀系数pi1为：
%%%%%公式7
%其中f(n)是关于竞争进程数的线性函数，受轮循时间大小和切换进程开销决定。freq是特定设备CPU频率关于温度的降频函数。 f(n)函数可在训练前离线快速测量并拟合， freq函数可通过cpu的DVFS策略感知。
%每层的访存时延主要受该层的访存量和访存带宽的影响。访存时延主要受缓存命中率影响。基于缓存命中率φ、缓存cache带宽bcache和内存DRAM带宽bdram，访存膨胀系数pi_2为：
%%%%%公式8
%因此，第l层的运行时延和离线时延关系为：
%%%%%公式9
%其中，N^l 和M^l 分别为第l层的浮点运算次数和访存量， $\delta _M$和$\delta _F$分别为单位访存时间和单次浮点运算时间。可以发现，由于计算膨胀系数和访存膨胀系数从浮点运算和内存带宽两个方面独立地影响计算时延和访存时延，在硬件条件动态变化时，不同层的运行时延变化的倍数并不相同。计算密度（cite：roofline model）是一个层或网络的重要指标，为浮点运算次数和访存量之比，即xx/xx（写公式）。公式9可以看出，层的计算密度越高（例如卷积层），运行时延受计算膨胀系数影响越大；层的计算密度越低（例如激活层），运行时延受访存膨胀系数影响越大。此外，相同类型层的计算密度也可能不同，如图xx所示。需要说明的是，尽管激活层等没有权重不参与更新，但依然需要参与反向传播计算梯度，因此也需要考虑在层时延范围内。
%在实际部署SwiftTTA时，需要首先在设备空闲条件下测量静态层时延。当设备实际运行时，根据当前硬件条件计算膨胀系数，从而得到当前设备状态下的层运行时延。通过对层运行时延的动态建模，能够在硬件条件实时发生变化而导致不同层由于计算密度不同而发生不同程度的时延变化时，为稀疏更新搜索算法提供准确的层时延信息，从而使实际运行时延符合预期加速效果。

\subsection{Tensor saving and reforwarding}
%在反向传播后，模型中被选定的层集合更新自身权重，未被选定更新的层的权重则和第一次前向传播时保持相同。因此在两次前向传播的输入数据相同的情况下，如果前n层未发生更新，那么前n层的计算在第二次前向传播中和第一次前向传播中相同。为了避免第二次前向传播中的冗余计算，SwiftTTA设计了tensor save-load机制。如图xx所示，在反向传播开始前，将首个更新层（第四层）的输入激活张量从梯度计算图中剥离（detach）并保留。在backward释放计算图后，加载中间激活并直接从模型第四层开始第二次前向传播计算。
%可以发现稀疏更新的策略不但会直接影响到反向传播，还会间接影响到第二次前向传播。因此，我们将第二次前向传播的时延合并到稀疏更新策略搜索时的优化目标，如公式0所示。首个更新层的位置越靠后，tensor save-load能够减少的冗余时延就越多。



==> body/others/design_eng.tex <==


\subsection{Overview}
In this section, we will first give an overview of SwiftTTA, then elaborate its each work stage.

%\textbf{Design goal}
%设计目标：SwiftTTA的目标是在给定数据流预测帧率需求的情况下最大化模型的测试时适应精度。在移动部署环境中，帧率需求通常由算法开发人员固定，或根据场景切换而在运行时动态调整。
%SwiftTTA基于稀疏更新方法，通过调整参与模型适应的层集合来调整模型适应过程中时延的bottleneck部分——BP，并同时利用tensor save-load机制调整第二次前向传播的时延，从而实现对数据流预测帧率的灵活控制。这一问题被表述为如下约束优化问题：
%%%%%公式0
%$$
%\max\text{\ }\vec{S}_t\cdot \vec{A}_t\ \ \ s.t.\ B_t\le \phi \cdot \left[ T_{t}^{f}+f_1\left( \vec{S}_t,t_b \right) +f_2\left( \vec{S}_t,t_{re} \right) \right] 
%$$
%其中xx是xx。
%为了在满足预测帧率的条件下最大化模型适应的精度收益，需要选择最重要的层集合参与更新，因此需要评估每层如果参与更新，预期带来的精度收益和时延成本。然而相比离线训练，模型在预测实时数据流时适应会产生数据偏移和硬件状态实时发生未知变化的问题，因此SwiftTTA的关键设计包括两个具有实时性的layer profiler——layer accuracy benefit profiler（4.3节）和layer latency overhead profiler（4.4节）。此外，SwiftTTA还通过tensor saver-loader机制进一步减少了未参与更新更新层带来的冗余Reforward时延，如4.5节所示。

\textbf{Design goal: }The goal of SwiftTTA is to maximize the test-time adaptation accuracy of the model while meeting the specified frame rate requirements for a given data stream. In mobile deployment environments, frame rate requirements are typically fixed by algorithm developers or dynamically adjusted at runtime based on scene changes.
SwiftTTA is based on sparse update methods and adjusts the set of layers involved in model adaptation to modify the bottleneck component of latency in the adaptation process, which is the backpropagation (BP). It also utilizes a tensor save-load mechanism to adjust the latency of the second forward pass, allowing for flexible control over the frame rate of data stream predictions. This problem is formulated as the following constrained optimization problem:
$$\max\text{\ }\vec{S}_i\cdot \vec{A}_t\ \ \ s.t.\ B_t\le \phi \cdot \left[ T_{t}^{f}+f_1\left( \vec{S}_t,l_{t}^{b} \right) +f_2\left( \vec{S}_t,l_{t}^{re} \right) \right] $$
To maximize the accuracy gains of model adaptation while meeting the frame rate requirements, it is necessary to select the most crucial set of layers for updating. This requires assessing the expected accuracy gains and latency costs for each layer if they were to participate in updates. However, compared to offline training, model adaptation during real-time data stream prediction introduces challenges related to data shift and the real-time unknown changes in hardware status. Therefore, the key design elements of SwiftTTA include two real-time layer profilers: the layer accuracy benefit profiler (Section 4.3) and the layer latency overhead profiler (Section 4.4). Additionally, SwiftTTA further reduces redundant reforward latency introduced by layers that are not updated through the tensor saver-loader mechanism, as shown in Section 4.5.


%
%Workflow。如图xx所示，SwiftTTA分三个阶段完成模型的适应和预测。
%\begin{itemize}
    %\item \textbf{Forward stage}. 
    %（1）在Forward stage，SwiftTTA对当前批次数据执行前向传播计算并实时完成对模型每层精度和时延信息的更新。首先，layer accuracy benefit profiler基于层间激活实时生成当前批次数据的分布统计信息并计算和历史数据分布间的KL-divergence；layer latency overhead profiler基于当前硬件状态（包括计算设备温度、系统竞争进程数和缓存命中率）和理想环境下每层的静态时延更新layer latency overhead。   
    %\item \textbf{Backward stage}. 
    %（2）在Backward stage，SwiftTTA搜索需要更新的层并完成对模型的部分反向传播计算。首先基于forward stage更新的层信息执行搜索，得到针对当前批次数据的层更新策略。随后在计算图中保留第一个更新层的激活后，根据层更新策略执行部分反向传播计算图，完成适应。
    %\item \textbf{Reforward stage}. 
    %（3）在Reforward stage，SwiftTTA读取保存的激活，并对适应后的模型重新执行部分前向传播过程，完成预测。
%\end{itemize}

\begin{figure*}[t]
  \centering
  \includegraphics[width=.9\textwidth]{figure/Swift-workflow.pdf} 
  \caption{}
  \label{fig:overview_1}
  \vspace{-2mm}
\end{figure*}

\textbf{Workflow}. As shown in Figure XX, SwiftTTA consists of three stages to accomplish model adaptation and prediction.
\begin{itemize}
    \item \textbf{Forward stage}.In the Forward stage, SwiftTTA performs forward pass computations on the current batch of data and updates the accuracy and latency information for each layer in real-time. First, the layer accuracy benefit profiler generates real-time distribution statistics for the inter-layer activations based on the current batch of data and calculates the KL-divergence between this distribution and the distribution from historical data. The layer latency overhead profiler, on the other hand, utilizes current hardware conditions, including computational device temperature, the number of competing processes in the system, and cache hit rates, to update the layer latency overhead for each layer based on their static latencies in an ideal environment. 
    \item \textbf{Backward stage}.In the Backward stage, SwiftTTA searches for the layers that need to be updated and performs partial backpropagation calculations for the model. First, it performs a search based on the layer information updated in the Forward stage to determine the layer update strategy tailored to the current batch of data. Subsequently, it retains the activations of the first updated layer in the computation graph and executes a partial backpropagation calculation according to the layer update strategy to complete the adaptation.
    \item \textbf{Reforward stage}.In the Reforward stage, SwiftTTA reads the saved activations and re-executes a partial forward pass process on the adapted model to complete the prediction.
\end{itemize}



\subsection{Tensor saving and reforwarding}
%在反向传播后，模型中被选定的层集合更新自身权重，未被选定更新的层的权重则和第一次前向传播时保持相同。因此在两次前向传播的输入数据相同的情况下，如果前n层未发生更新，那么前n层的计算在第二次前向传播中和第一次前向传播中相同。为了避免第二次前向传播中的冗余计算，SwiftTTA设计了tensor save-load机制。如图xx所示，在反向传播开始前，将首个更新层（第四层）的输入激活张量从梯度计算图中剥离（detach）并保留。在backward释放计算图后，加载中间激活并直接从模型第四层开始第二次前向传播计算。
%可以发现稀疏更新的策略不但会直接影响到反向传播，还会间接影响到第二次前向传播。因此，我们将第二次前向传播的时延合并到稀疏更新策略搜索时的优化目标，如公式0所示。首个更新层的位置越靠后，tensor save-load能够减少的冗余时延就越多。
After backpropagation, the selected set of layers in the model updates their own weights, while the layers not selected for updates retain their weights from the first forward pass. Therefore, if the first 'n' layers remain unaltered, their computations in the second forward pass, when the input data is the same as in the first pass, are identical to those in the first forward pass. To avoid redundant computations in the second forward pass, SwiftTTA employs a tensor save-load mechanism. As illustrated in Figure XX, before the start of backpropagation, the input activation tensor for the first updated layer (the fourth layer) is detached from the gradient computation graph and preserved. After releasing the backward graph, the intermediate activations are loaded and used directly to compute the second forward pass starting from the fourth layer of the model.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.4\textwidth]{figure/tensor save load.pdf}
  \caption{}
  \label{fig:intra_para}
  % \vspace{-3mm}
\end{figure}

It is noteworthy that the strategy of sparse updates not only directly affects backpropagation but also indirectly influences the second forward pass. Hence, we incorporate the latency of the second forward pass into the optimization objective during the search for sparse update policies, as shown in Formula 0. The farther back the position of the first updated layer, the more redundant latency can be reduced by the tensor save-load mechanism.


==> body/others/design_v2.tex <==
%在本节中，我们首先根据TTA的

% \subsection{Optimizing Goal}

% ！！！！！！！！！！！！！！！！！！！！！！！！！！
%整section的主要问题是优化目标的缺失？，而不是证明或者构建方程。
%你需要清晰地用公式表达出：需要更新的部分究竟在哪一部分？
%其他的有关“是否更新或者更新机会”的部分，是上一节的内容，这部分的公式应该放在上一节，这部分公式正是承接上一节展开的

%To optimize the latency of device-side testing adaptation, we first need to model the latency of a complete adaptation process and analyze the key components and influencing factors of the latency. Under the ideal offline mobile device condition, for the input $x_t$ at time $t$, a complete adaptation process consists of three stages: forward, backward, and reforward, as shown in the figure. Forward propagation calculates inter-layer activations based on $x_t$; backward propagation calculates gradients based on inter-layer activations and updates model parameters; reforwarding gives the final prediction based on the optimized model parameters.

%Therefore, at time t, the total latency of an adaptation process consists of three parts, as Eq.~\ref{d1},
%为了优化设备端测试时适应的时延，我们需要首先对一次完整适应过程的时延进行建模，并分析时延的关键组成部分和影响因素。在离线的理想移动端设备条件下，对于t时刻的输入xt，一次完整的适应过程包括三个阶段：forward、backward和reforward，如图xx所示。前向传播基于xt计算层间激活；反向传播基于层间激活计算梯度并更新模型参数；reforward基于优化后的模型参数给出最终预测结果。
%因此，在时刻t,一次适应过程的总时延由三部分组成：

Compared with standard data flow inference, testing adaptation adds the process of online updating, namely backward and reforward. Therefore, optimizing the latency of backward and reforward is crucial to improve the throughput (fps) of data flow inference. In addition, the more dynamic device resources and hardware conditions during online model adaptation bring greater dynamicity to the actual execution latency. To achieve the expected acceleration effect of the sparse updating strategy, it is necessary to predict the actual execution latency based on offline latency and real-time device resource parameters. Therefore, our final optimzing goal, as Eq.~\ref{r3},
\begin{equation} \label{r3}
    \max\text{\,\,}\vec{S}_t\cdot \vec{A}_t\,\,\,\,\,\,\ \ s.t.\ \ b_t\le \phi \cdot \left[ T_{for}+T_{back}^{t}+T_{refor}^{t} \right]
\end{equation}
where $T$ is XXX.

%其中$T_{for}$,$T_{back}$,$T_{refor}$分别是forward,backward和reforward在理想环境下的时延，$\varphi _t$是时刻t时设备的资源参数,f函数基于理想时延和实时硬件资源参数预测实际执行时延。如图xx（a）所示，反向传播需要同时计算参数梯度$\delta w_l$和输入激活梯度$\delta x_l$：
% $$
% T_{back}=\sum_{b=1}^B{\sum_{l=1}^L{\left( t_{\delta w_l}+t_{\delta x_l} \right)}}
% $$
%而forward和reforward只需要计算每层前向输出：
% $$
% T_{for}=T_{refor}=\sum_{b=1}^B{\sum_{l=1}^L{t_{fw_l}}}
% $$
%因此反向传播的时延是整个适应过程的bottleneck，如图xx（b）所示。相比于标准数据流推理而言，测试时适应增加了在线更新的过程，即backward和reforward。因此优化backward和reforward的时延对提升数据流推理的吞吐量（fps）十分重要。此外，模型在线适应时更加动态的设备资源和硬件条件也给实际执行时延带来了更大的动态性，为了完成稀疏更新策略的搜索和预期加速效果，需要基于离线时延和实时设备资源参数$\varphi _t$预测实际执行时延。

% \subsection{Chameleon Framework}

%\textbf{Design goal}
%设计目标：Chameleon的目标是在满足数据流推理fps目标的条件下最大化模型的在线适应精度收益。在移动部署环境中推理fps需求通常由算法开发人员固定，并在运行时随任务需求动态调整。
%对于时刻t的输入数据xt，Chameleon基于每层的精度重要性和实际运行时延，通过剪枝优化的动态规划算法完成稀疏更新策略$\vec{S}_t$的搜索。通过调整$\vec{S}_t$的大小，能够灵活控制backward时延。随后在reforward中，Chameleon利用tensor save-reload schedule复用forward的计算以进一步优化reforward的计算时延。这可以被表述为如下约束优化问题：
%$$
%\max\text{\,\,}\vec{S}_t\cdot \vec{A}_t\,\,\,\,\,\,\ \ s.t.\ \ b_t\le \phi \cdot \left[ %T_{for}+T_{back}^{t}+T_{refor}^{t} \right] 
%$$
%其中$\vec{A}_t$,$\phi$是任务需要的推理fps,$b_t$是t时刻输入数据批次大小，$\vec{S}_t$是控制每一层是否参加本次更新的稀疏更新策略，T_{back}^{t}是基于$\vec{S}_t$策略的优化后反向传播时延, T_{refor}^{t}是基于$\vec{S}_t$策略的优化后reforward时延.
%例如对于六层NN模型的更新策略$\vec{S}_t=\left[ 0,0,1,0,0,1 \right]$, 链式计算的backward和reforward需要包含第一个更新层后的所有层。即
%$$
%T_{back}^{t}=\left[ 0,0,1,1,1,1 \right] \cdot \left[ l_{back}^{1},...,l_{back}^{6} \right] 
%$$
%$$
%T_{refor}^{t}=\left[ 0,0,1,1,1,1 \right] \cdot \left[ l_{refor}^{1},...,l_{refor}^{6} \right] 
%$$
%其中l_{back}^{i}和l_{refor}^{i}分别是第i层的反向传播和reforward时延。

% \noindent \textbf{Design goal}. 
To handle the above intractable problem, we present Chameleon.
It maximizes the model's online adaptation accuracy while satisfying the target data stream inference throughput. The throughput requirement for inference is typically fixed by algorithm developers or users and dynamically adjusted at runtime based on task demands.

%为了在达到推理fps目标的情况下最大化模型适应的精度收益，需要选择最重要的一部分层参与稀疏更新，因此准确预测每层参与更新带来的适应精度收益和额外时延成本至关重要。相比于静态环境下的离线训练，基于实时数据流的on-device在线适应的数据分布动态性和设备资源动态性，会分别给NN模型每一层的精度重要性和实际执行时延带来实时动态性。因此Chameleon的关键设计包括两个具有实时性的layer profiler——layer-wise accuracy-importance profiler（4.1节）和layer-wise latency-overhead profiler（4.2节）。Chameleon还通过设计与稀疏更新协同工作的三个子模块：经过剪枝优化的搜索算法、计算图节点修剪和tensor saver-loader机制,进一步降低了在线适应时延。

To maximize adaptation accuracy while achieving target inference throughput, it is crucial to select the most important subset of layers for sparse update. Therefore, accurately predicting the adaptation accuracy gain and additional latency cost for each layer participating in update is essential. Compared to offline training, the real-time dynamics of data distribution in on-device online adaptation based on real-time data streams and the dynamic device resources bring real-time dynamics to the accuracy importance and actual execution latency for each layer in NN models.

Therefore, Chameleon's key design includes two real-time layer profilers: 
the layer-wise accuracy-importance profiler (Sec.~\ref{}) and the layer-wise latency-overhead profiler (Sec.~\ref{}). 
Chameleon further reduces online adaptation latency by designing three sub-modules that work in synergy with sparse updates: a pruning-optimized search algorithm, computation graph node pruning, and a tensor saver-loader mechanism (Sec.~\ref{}).

%随后使用经过剪枝优化的动态规划算法，基于评估结果完成更新策略$\vec{S}_t$的搜索，并基于策略对不参与更新的计算图梯度节点进行修剪，实现稀疏反向传播和更新，如5.1节所示。最后，Chameleon还设计了tensor saver-loader机制，通过复用没有参与更新的层的前向传播计算结果，降低了reforward的冗余计算时延，如5.2节所示。

Subsequently, using a pruning-optimized dynamic programming algorithm, Chameleon performs a search for the update strategy \(\vec{S}_t\) based on the evaluation results. It prunes the computation graph gradient nodes that are not involved in the update according to the strategy, enabling sparse backward propagation and updates, as depicted in Sec.~\ref{}. Finally, Chameleon also introduces a tensor saver-loader mechanism, which reduces redundant computation latency in reforward by reusing the forward propagation results of layers that were not updated, as explained in Sec.~\ref{}.

%\textbf{Workflow}. 如图xx所示，Chameleon分三个阶段完成模型的适应和inference。
%\begin{itemize}
    %\item \textbf{Forward stage}. 
    %（1）在Forward stage，Chameleon对t时刻输入数据$x^t$执行前向计算并实时完成对模型每层精度重要性和执行时延的更新。Accuracy-importance profiler基于$x^t$产生每层激活的多阶分布统计和历史累计分布统计间的KL-divergence大小来评估每层更新的必要性；Latency-overhead profiler基于当前设备资源（包括主频、竞争进程和缓存命中率）和layer-wise offline latency预测layer-wise online latency。
    %\item \textbf{Backward stage}. 
    %（2）在Backward stage，Chameleon搜索稀疏更新策略$\vec{S}_t$并完成模型的稀疏反向传播和更新。首先基于基于评估结果使用经过剪枝优化的动态规划算法完成对更新策略$\vec{S}_t$的搜索。随后基于$\vec{S}_t$对不参与更新的计算图梯度节点进行修剪，在将首个更新层的输入激活$x^r$从计算图中修剪并保存在内存中，最后执行稀疏反向传播和更新。
    %\item \textbf{Reforward stage}. 
    %（3）在Reforward stage，Chameleon读取backward中保存的激活$x^r$，通过重用未更新的层的forward计算结果，重新执行更新后的模型的部分前向计算过程，完成数据流推理。
%\end{itemize}

As shown in Figure \ref{fig:Swift-workflow}, Chameleon completes the adaptation and inference of the model in three stages.
\begin{itemize}
    \item \textbf{Forward stage}. 
    In the Forward stage, Chameleon performs forward computation on the input data \(x^t\) at time \(t\) and dynamically updates the accuracy importance and execution latency for each layer in real-time. The Accuracy-Importance Profiler evaluates the necessity of updating each layer based on the KL-divergence between multi-order distribution statistics of the activations generated by \(x^t\) and historical cumulative distribution statistics. The Latency-Overhead Profiler predicts layer-wise online latency based on current device resources, including clock frequency, competing processes, and cache hit rates, using layer-wise offline latency as a reference.
    \item \textbf{Backward stage}. 
    In the Backward stage, Chameleon searches for the sparse update strategy \(\vec{S}_t\) and completes sparse backward propagation and updates for the model. First, using a pruning-optimized dynamic programming algorithm based on the evaluation results, it searches for the update strategy \(\vec{S}_t\). Then, based on \(\vec{S}_t\), it prunes the computation graph gradient nodes that are not involved in the update. The input activation \(x^r\) from the first updated layer is pruned from the computation graph and stored in memory. Finally, sparse backward propagation and updates are executed.
    \item \textbf{Reforward stage}. 
    In the Reforward stage, Chameleon reads the saved activation \(x^r\) from the backward stage. By reusing the forward computation results of layers that were not updated, it partially re-executes the forward computation process for the updated model and completes the data stream inference.
\end{itemize}

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.96\linewidth]{figure/Swift-workflow.pdf}
  \caption{TODO}
  \label{fig:Swift-workflow}
\end{figure*}






==> body/others/introduction.tex <==
% Introduction

\TODO[The main challenge of achieving wall-clock time speedup is how to precisely profile the training times of different tensor selections.]











% 问题背景和现状：Background
% 随着智能物联网的普及，深度神经网络被广泛部署在移动设备上，例如自动驾驶~\cite{},视频安防~\cite{},缺陷检测~\cite{}等。
%（云边训练的一般范式）由于网络的训练成本远大于推理成本，网络首先在云端进行预训练，在终端执行推理。
% 然而，当边端场景
% 采用云边协同的范式完成 
%（范式之下的问题）云端训练数据分布往往无法覆盖移动端所有的部署环境，因此当模型部署后面临未见过的新场景时，推理精度会发生大幅下降~\cite{}。因此，模型在移动设备部署后通常还需要重新适应新场景以恢复推理精度。

%Related Works

%Currently, 现有的适应方案需要提前采集并标注新场景下的大量数据，随后离线进行多轮重训练（which通常持续数个小时~\cite{et，melon}）。

%1. 然而这种方式需要提前收集新场景数据并人工标注，但收集和标注的时间和成本非常昂贵，并且在移动端上通常难以实现，例如自动驾驶模型无法预知第二天场景的天气和所处环境。
%2. 此外，由于模型有限的表达能力和场景到达的次序性，模型适应一个场景后当切换到一个新场景时，需要重新离线训练。这在无人机探测、自动驾驶等场景切换速度以分钟为单位的任务中可能会造成非常高的开销，甚至无法正常执行任务。

1.人工成本高(获得label开销大)
1.1.标注时间长->等他标注好->等的时候没办法retrain model->影响模型domain generation (排100个人帮你可以吗？ -> ）

2.Online model -> 适应 多样化的 随机的 现实（在线）场景 是一个挑战。而之前的方法，无法及时（immediately）泛化（adapt to）到新的场景。

3.变化随机，以至于难以预测 -> 

4.

%Problems(current soluiton's problem -> problem you need to solve)
%测试时适应（TTA）是近年域适应为了解决访问源域带来的隐私问题而提出的一种模式。我们发现TTA模式也适用于快速变化移动端场景下的模型适应，TTA不需要提前收集任何新场景的数据，而是当模型在新场景执行推理任务时，仅基于当前批次实时输入数据完成模型的在线适应后再推理该批次数据。因此测试时适应相比离线重训练能够更灵活地适应移动端场景，并且测试时适应和重训练并不冲突，能够耦合使用以进一步提高精度：在部署前基于训练数据完成通用性适应，在执行预测任务时对当前输入样本进行针对性适应。

%已有TTA方法的不足：
%然而现有的TTA方法关注如何提高无监督训练的可信度和训练精度并面向服务器设备展开验证。当这些方法部署在算力有限的移动设备上时会造成较高的适应时延，严重影响了设备推理的速度。

%为什么在TTA中我们要用稀疏更新技术实现加速
%为了减少模型适应的时延，我们应用稀疏更新技术来减少设备端测试时适应的时延。这是因为在调研后发现稀疏更新能够在减少适应时延的同时减轻连续无监督训练中的错误累计，并且几乎不需要修改就能够和其他训练优化技术如计算卸载和量化等耦合使用。

%已有稀疏更新方法的不足： 
%静态稀疏更新方法~\cite{}离线评估层精度收益和搜索稀疏更新策略，并应用于随后的整个离线训练过程。但这种固定稀疏更新方案的方法会导致模型学习能力有限或训练时间增加~\cite{}。
%现有动态稀疏更新方法~\cite{}面向离线重训练而设计，在离线训练时每隔数个epoch动态重新评估层精度收益以提高训练精度，但每次评估所需的层梯度需要依赖完整的反向传播计算得到，时延成本较高。因此动态稀疏更新通过减少评估次数以降低评估过程的总开销，但这仅在适应单个场景（数据分布相同）的情况下适用，当场景不断切换时，需要频繁地评估层精度收益，这会导致非常高的评估时延。此外，动态稀疏更新基于离线测量的层时延搜索稀疏加速策略，这在离线训练时的空闲设备状态下通常能够实现预期加速。但TTA通常在设备忙碌时运行，硬件条件的高动态性会导致层的实际运行时延和离线测量时延产生较大差异，从而造成不准确的时延加速效果。

%方法目标：Ours Method (Facing the problems) we do...
%我们的目标是在连续场景的测试时适应条件下基于稀疏更新技术实现对模型适应的灵活加速。
%第一，稀疏更新需要准确的层精度收益来保证搜索得到的稀疏更新策略对精度有效的提升。层精度收益和当前输入数据的分布有关~\cite{}。针对当前输入数据实时评估层精度收益具有挑战性，因为层精度收益的评估通常依赖离线微调~\cite{tte}或梯度~\cite{et}数据，这会导致大量的额外开销。因此我们从原始适应过程中已有的输入数据和中间激活入手，从每层当前激活数据和历史激活数据间分布差异的显著性来评估更新每层可能带来的精度收益。
%第二，稀疏更新需要准确的层运行时延来保证搜索得到的稀疏更新策略能够实现对时延的预期加速。每层实际运行时延和当前系统环境相关。现有稀疏更新方法直接利用离线测量的层时延进行搜索，因为离线训练（通常在深夜）和离线测量时延的系统环境相似。然而TTA在设备执行预测任务时在线运行，这意味着更多的设备端竞争进程（例如无人机控制程序，手机其他应用程序）可能导致系统环境和离线测量的环境差异较大，因此静态层时延不能准确反映当前层运行时延。为了应对这一挑战，我们对层的静态时延和实际运行时延间的关系进行了建模，并在TTA运行时基于设备当前系统环境分析每层的实际运行时延，从而保证稀疏更新策略能够在动态设备条件下实现预期加速。
%第三，在测试时适应中，模型适应结束后需要再次推理以获得更准确的预测结果。我们发现稀疏更新避免了一些层参数的更新，再次推理时一些未更新的层有机会复用第一次推理时的激活从而避免重复计算。我们发现第二次推理能够节省的时延取决于稀疏更新中第一个更新层的位置。因此我们设计了与稀疏更新协同的tensor save-load机制并将第二次推理时延加入到稀疏更新的搜索目标中，进一步降低了测试时适应的时延。



\textbf{Contributions} are summarized as following.
\begin{itemize}
%我们提出了Chameleon，一个基于稀疏更新技术和与之协同的tensor save-load机制共同降低设备端适应时延的框架。据我们所知，Chameleon是第一个在连续测试时适应场景下面向移动端设备实现灵活加速适应的工作。
%我们基于分布对齐的思想，提出了一种能够对输入数据实时评估层精度收益的方法。
%我们构建了动态时间模型，能够基于层静态时延和当前设备的系统环境，实时分析层的实际运行时延。
%experiments效果
\item{experiments}
\end{itemize}

==> body/others/method_1.tex <==
\subsection{Layer-wise accuracy-importance profiler}
%为了maximize稀疏更新策略带来的精度收益，需要准确evaluate每层的精度重要性，并选取最重要的一部分层参与更新。
%如\ref{Dynamic data distribution.}所述，每层的精度重要性在不同的数据偏移环境下会发生改变。在测试时适应时，实时数据流的分布未知并且实时变化，因此需要频繁在当前输入数据的潜在分布下进行层精度重要性的评估。现有的稀疏更新方法逐步撤销每层更新并对比精度变化~\cite{}或基于完整的反向传播计算和梯度累加~\cite{}来评估层精度重要性，频繁执行评估会带来很高的计算成本。

%我们将从模型在移动数据偏移场景下精度发生下降的根本原因入手，探索每层更新能够带来的潜在精度收益。此外，我们还将尽可能地重用已有数据，以避免额外的计算成本。         
%在TTA场景下，模型预测精度下降的根本原因是新场景（模型还未适应）的数据分布与历史场景（模型已经适应）的数据分布之间的差异较大，超出了模型当前的预测范围（即泛化能力）。更新模型可以扩展模型参数的可预测范围，减小两个场景下数据分布间的距离（即对齐分布差异），以适应新的数据分布~\cite{域适应工作}。
%因此我们从分布对齐的角度出发，通过计算当前场景的数据分布是否在每层参数的可预测范围内来表示每层参数在当前场景下更新后对模型适应精度的影响。
%对于在某层参数可预测范围内的不同数据，该层输出的分布是稳定的。然而当数据逐渐远离可预测范围时，该层输出的分布会出现越来越显著的差异。
%因此我们用每层当前输出的分布和历史输出的分布间的差异来表示当前数据是否在每层的可预测范围内。
%在新场景数据的未知分布下，若某层当前输出的分布与历史输出的分布接近，则表明该层能将当前数据映射到已知分布，具有更强的泛化性。模型的每一层具有不同的泛化能力，在特定的输入分布下，泛化性强的层应适度更新，以避免错误累积和过拟合；而泛化性较弱的层则应大幅更新，以充分适应新的数据分布。
%4-10精简精简精简精简
%stop here

%给定一个深度网络\(f\left( x;\theta \right) \)，其中 \(x\) 是输入图像，\(θ\) 是模型参数。$H$是模型已经适应的历史分布，$C_t$是当前时刻输入数据的分布。为了保证评估方法的通用性和便捷性，我们不对网络架构或云端训练过程作出任何假设。为了减小提取数据分布的成本，我们仅限于用统计数据来表征分布。现有方法通常通过提取样本高阶矩来获取统计信息\cite{HoMM: Higherorder Moment Matching for Unsupervised Domain Adaptation,Central Moment Discrepancy (CMD) for Domain-Invariant Representation Learning.}，然而在移动环境下我们的数据批次可能较小，因此高阶矩难以提取到准确的数据分布。为了平衡统计信息的准确性和计算成本，并使SwiftTTA能够实现小批量在线适应，我们分别对第\(l\)层输出\(o_l\)，并提取channel-wise的means \(\mu _{l,c}\):
$$
\mu _c\left( f_l\left( x \right) \right) =\frac{1}{N}\sum_{i=1}^N{f_{l,c}^{i}\left( x \right)}
$$
%and variances \(\sigma _{l,c}^{2}\):
$$
\sigma _{c}^{2}\left( f_l\left( x \right) \right) =\frac{1}{N}\sum_{i=1}^N{\left( f_{l,c}^{i}\left( x \right) -\mu _c\left( f_l\left( x \right) \right) \right) ^2}
$$
%通过计算每个通道的\(\mu _{l,c}\)和\(\sigma _{l,c}^{2}\)并将它们连接，我们得到第\(l\)层输出对于输入分布$C_t$的分布表征\(D_{l}^{t}\)：
$$
E_{l}^{t}=\left[ \mu _1\left( f_l\left( x \right) \right) ,\ \sigma _{1}^{2}\left( f_l\left( x \right) \right) ,\ .\ .\ .\ ,\ \mu _c\left( f_l\left( x \right) \right) ,\,\,\sigma _{1}^{2}\left( f_l\left( x \right) \right) \right] 
$$
%分布表征\(D_{l}^{t}\)是由\(o_l\)逐通道的均值和方差组成的K维向量。如图xx所示，以图像数据为例，这种分布表征能够有效表示当前图像的风格与语义信息。我们计算第\(l\)层当前输出的分布表征\(D_{l}^{t}\)和历史输出的分布表征\(D_{l}^{H}\)间的KL-divergence来表示第\(l\)层的精度重要性\(a_l\):
$$
a_l=D_{KL}\left( E_{l}^{H}\lVert E_{l}^{t} \right. \right) =\sum_{b=1}^B{E_{l,b}^{H}\log \frac{E_{l,b}^{H}}{E_{l,b}^{t}}}
$$
%该指标反映了对于第\(l\)层，当前数据的分布偏离模型可预测范围的程度，偏离程度越大，更新第\(l\)层带来的精度收益就越高。由于模型需要不断适应新的场景，因此代表模型已经适应的历史分布$H$也需要随着模型的适应而不断更新。在连续场景的适应中，我们利用an exponential moving average technique来逐渐更新历史分布表征：
$$
E_{l}^{t}=\alpha E_{l}^{t-1}+\left( 1-\alpha \right) E_{l}^{H}
$$
%其中xx ∈ [0, 1]。
%为了在缺少数据标签的情况下训练模型，现有测试时适应方法通常最小化模型最后一层输出的熵来增强模型的置信度。但这种方法忽略了数据本身包含的分布信息，为了充分利用小批次数据，并使层精度重要性能够更准确的反映层的更新必要性，我们以减小模型每层的当前输出和历史输出之间的分布表征距离作为优化目标，并设计损失函数：
$$
L=\sum_{i=1}^I{D_{KL}\left( E_{i}^{H}\lVert E_{i}^{t} \right. \right)}
$$

%由于逐个通道而非逐个参数提取提取一阶统计量和二阶统计量，并且重用了forward的计算结果，我们提出的层精度重要性评估方法是计算友好和内存友好的。对于vgg16，resnet50和mobilenetv2而言，评估batchsize为16的数据的层精度重要性的计算开销分别约为推理的xx%，xx%和xx%。储存在设备中的历史数据的分布表征与层数和通道数相关。对于resnet50而言，$H$的大小通常在xxKB左右。此外，如果将分布提取过程和forward并行计算能够进一步减小评估带来的额外开销。


\subsection{Layer-wise latency-overhead profiler}
%选择更多重要的层参与更新能够带来更显著的适应精度收益，但也会带来更高的适应时延。为了确保模型的适应时延满足给定约束，我们需要基于每一层的准确执行时延来预测稀疏更新方案的总时延。
%如\ref{Dynamic hardware condition.}所述，每层的实际运行时延在不同的硬件条件下会发生改变。测试时适应通常在设备完成预测任务时在线进行，此时分配给每个应用程序的硬件资源是高度动态的。这意味着适应进程需要和忙碌设备上更多的其他进程同时竞争设备资源，例如无人机的控制程序、手机的应用程序，这给每层的实际执行时延带来了更多的不确定性。
%为了准确评估动态硬件条件下的层时延，需要首先分析影响层时延的各个组成部分的硬件条件因素。在深度模型的推理和训练过程中，每一层在设备理想环境下的总时延主要由计算时延和访存时延组成：\(T_{off}^{l}=T_{MAC}^{l}+T_{MEM}^{l}\)。
%当设备实际运行时，每一层的计算时延和访存时延受当前的主频和cache-hit-rate等不同因素影响而变化。因此第\(l\)层的在线运行时延T_{on}^{l}在运行环境下与理想环境下的离线时延T_{off}^{l}关系可建模为：\(T_{on}^{l}=\pi _1\cdot T_{F}^{l}+\pi _2\cdot T_{M}^{l}\)。其中\(pi_1\)，\(pi_1\)分别为计算时延和访存时延在实际运行条件下的相比于理想环境下的时延的增加倍数，我们称之为计算膨胀系数和访存膨胀系数。

%每层的计算时延主要受该层的浮点运算次数和设备单位时间内能够执行浮点运算次数的影响。对于相同层和相同设备而言，影响单位时间内能够执行该层的浮点运算次数的因素主要包含竞争进程数和硬件温度（例如CPU、GPU）。%\textbf{竞争进程数}：资源受限的移动设备通常依赖CPU或GPU完成计算。以CPU为例，设备操作系统内核（如Linux）默认采用Round Robin scheduling（RR）公平调度计算进程。导致当竞争进程数上升时，当前计算进程的等待时间也会随之上升。%\textbf{硬件温度}：当设备CPU温度升高时，动态电压频率缩放（DVFS）会通过降低主频控制功耗。这会导致当前计算进程的计算时间上升。
%因此，竞争进程数为\(n\)，CPU或GPU温度为\(tem_on\)时，计算膨胀系数\(pi_1\)为：
$$
\pi _1=\frac{freq\left( tem_{off} \right)}{freq\left( tem_{on} \right)}\cdot \left[ 1+f\left( n \right) \right] 
$$
%其中\(f\left( n \right)\)是关于竞争进程数的线性函数，受轮循时间大小和切换进程开销决定。\(freq\)是特定设备CPU频率关于温度的降频函数。 \(f\left( n \right)\)函数可在训练前离线快速测量并拟合， \(freq\)函数可通过CPU或GPU的DVFS策略感知。

%每层的访存时延主要受该层的访存量和访存带宽的影响。访存时延主要受缓存命中率影响。基于缓存命中率\(\varphi\)、缓存带宽\(b_cache\)和内存DRAM带宽\(b_dram\)，访存膨胀系数\(pi_2\)为：
$$
\pi _2=\frac{\left[ \varphi \cdot b_{cache}+\left( 1-\varphi \right) \cdot b_{dram} \right]}{b_{cache}}
$$
%因此，第\(l\)层的运行时延和离线时延关系为：
$$
T_{on}^{l}=\frac{\pi _1\cdot \eta _l+\pi _2}{\eta _l+1}\cdot T_{off}^{l}
$$

$$
\eta _l=\frac{T_{F}^{l}}{T_{M}^{l}}=\frac{N^l}{\delta _M}\cdot \frac{\delta _F}{M^l}
$$

%其中，\(N^l\) 和\(M^l\) 分别为第\(l\)层的浮点运算次数和访存量， $\delta _M$和$\delta _F$分别为单位访存时间和单次浮点运算时间。

%可以发现，由于计算膨胀系数和访存膨胀系数从浮点运算和内存带宽两个方面独立地影响计算时延和访存时延，在硬件条件动态变化时，不同层的运行时延变化的程度并不相同。计算密度（cite：roofline model）是一个层或网络的重要指标，为浮点运算次数和访存量之比，即xx/xx（写公式）。公式9可以看出，层的计算密度越高（例如卷积层），运行时延受计算膨胀系数影响越大；层的计算密度越低（例如激活层），运行时延受访存膨胀系数影响越大。此外，相同类型层的计算密度也可能不同，如图xx所示。需要说明的是，尽管激活层等没有权重不参与更新，但依然需要参与反向传播计算梯度，因此也需要考虑在层时延范围内。

%在实际部署SwiftTTA时，需要首先在设备空闲条件下测量静态层时延。当设备实际运行时，根据当前硬件条件计算膨胀系数，从而得到当前设备状态下的层运行时延。通过对层运行时延的动态建模，能够在硬件条件实时发生变化而导致不同层由于计算密度不同而发生不同程度的时延变化时，为稀疏更新搜索算法提供准确的层时延信息，从而使实际运行时延符合预期加速效果。

==> body/others/method_1_v2.tex <==
%由于不同网络层级在更新过程中性能和时延的普遍差异。为了对网络的精度重要性和时延重要性实时评估，我们分别采用了两种不同的Profiler对网络的层进行实时监控。
Due to the general differences in performance and latency among different network layers during the update process, we adopted two different profilers to monitor the layers of the network in real-time.

\subsection{Accuracy-Importance Profiler (AIP)}
%如\ref{Dynamic data distribution.}所述，每层的精度重要性在不同的数据场景下会发生改变。在测试时适应时，实时数据流的分布未知并且实时变化，因此需要频繁在当前输入数据的潜在分布下进行层精度重要性的评估。但是，现有的稀疏更新存在两个问题:第一，现有方法逐步撤销每层反向传播并对比精度变化~\cite{}，或基于完整的反向传播计算获取每层梯度信息~\cite{}来评估层精度重要性，频繁执行评估会带来很高的计算成本。第二，现有方法需要依赖数据标签，基于正确的标签进行反向传播得到的梯度或精度变化才能够反映每层的精度重要性。在实时场景下，错误的伪标签会干扰精度重要性的评估。
As described in Section \ref{Dynamic data distribution}, the accuracy importance of each layer varies in different data scenarios. During test-time adaptation, the distribution of real-time data streams is unknown and constantly changing. Therefore, it is necessary to frequently evaluate the accuracy importance of each layer under the potential distribution of the current input data. However, existing sparse update methods have two issues. Firstly, these methods evaluate the accuracy importance of each layer by gradually freezing the update of each layer and comparing the accuracy change \cite{reference1}, or by calculating the gradient of each layer based on the backward of the whole model \cite{reference2}. Frequent evaluations result in high computational costs. Secondly, existing methods rely on data labels. Only the gradient or accuracy change calculated based on the correct label during the backward pass can represent the accuracy importance of each layer. In real-time scenarios, incorrect pseudo-labels can interfere with the evaluation of accuracy importance.

%为了解决上述问题，我们考虑到反向传播带来显著计算成本和易受错误伪标签干扰的影响，我们的Profiler仅基于输入数据而不依赖任何数据标签，通过对齐新旧数据的分布差异，减少了反向传播带来的时间成本，并避免了错误伪标签对评估结果的干扰。具体来说，由于在更新新场景时，模型各层的输出分布和历史场景下的输出分布会出现明显差异，超出模型的泛化范围，使得精度下降。因此当前数据下层输出的分布和历史输出的分布间的差异越大，该层需要参与适应的必要性越大，层重要性$a_l$越高。

In order to address the mentioned problems, we propose the profiler that only relies on input data without any labels, in order to reduce the computational cost brought by backward and avoid the interference of incorrect pseudo-labels. Specifically, when the model comes to a new scenario, layer's output distribution will differ from that in the historical scenarios significantly, which exceeds the model's generalization ability and causes a decrease in accuracy. Therefore, the larger the difference between layer's output distribution under current data and the distribution under historical data, the greater the degree to which the model's layers need to adapt, and the higher the layer importance $a_l$
Therefore, under the current data, the greater the difference between the distribution of layer outputs and the distribution of historical outputs, the greater the necessity for the layer to participate in adaptation, and the higher the layer importance $a_l$.

%为了保证评估方法的通用性和便捷性，我们不对网络架构或云端训练过程作出任何假设。给定一个深度网络\(f\left( x;\theta \right) \)，其中 \(x\) 是输入图像，\(θ\) 是模型参数。$H$是模型已经适应的历史分布，$C_t$是当前时刻输入数据的分布。在t时刻设备所处环境的数据下，我们的Profiler基于前向传播后每层的输出$f_l\left( x \right)$提取分布$E_{l}^{t}$，并和该层历史输出的分布计算KL-divergence来表示每一层在当前输入数据下更新的必要性，即精度重要性$a_l$:
To ensure the universality and convenience of the evaluation method, we don't make any assumptions about the network architecture or cloud training process. For any deep network \(f\left( x;\theta \right) \), where \(x\) is the input image and \(\theta\) is the model parameters. $H$ is the historical data distribution the model has adapted, and $C_t$ is the distribution of current input data $x_t$ at time \(t\). Our profiler extracts the distribution embedding $E_{l}^{t}$ based on layer's output $f_l\left( x \right)$ generated in forward and calculates the KL-divergence with the historical output distribution embedding $E_{l}^{H}$ to represent the necessity of updating each layer under the current input data, i.e., the accuracy importance $a_l$, as Eq.~\ref{m1-1},
\begin{equation}\label{m1-1}
    a_l=D_{KL}( E_{l}^{H}\lVert E_{l}^{t}) \\
=\sum_{b=1}^B{E_{l,b}^{H}\log \frac{E_{l,b}^{H}}{E_{l,b}^{t}}},
\end{equation} 
% where %%分布表征是基于第l层的输出$f_l\left( x \right)$逐通道提取得到的K维向量。该指标反映了对于第\(l\)层，当前数据的分布偏离模型可预测范围的程度，偏离程度越大，更新第\(l\)层带来的精度收益就越高。基于此，我们的评估方法通过避免反向传播计算，显著的减少了评估开销，同时也避免了依赖错误伪标签而带来的有偏评估。（图）
where \(E_{l}^{t}\) is a K-dimensional vector obtained by extracting channel-wise from the output of the \(l\)th layer $f_l\left( x \right)$. This indicator represents the degree to which the current data distribution deviates from the predictable range of the model for the \(l\)th layer. The greater the deviation, the higher the accuracy gain from updating layer \(l\). Only based on forward, our evaluation method significantly reduces the evaluation cost by avoiding the calculation of backward, and also avoids biased evaluation caused by relying on incorrect pseudo labels, as Fig.~\ref{}.

%为了得到数据分布\(E_{l}^{t}\)并减小提取过程的计算和存储开销，我们用具有代表性的统计量来表示完整数据分布。现有方法通常通过提取样本高阶矩来获取统计信息\cite{HoMM: Higherorder Moment Matching for Unsupervised Domain Adaptation,Central Moment Discrepancy (CMD) for Domain-Invariant Representation Learning.}，然而在移动环境下输入数据batch size可能较小，因此高阶矩难以提取到准确的数据分布。我们分别对第\(l\)层输出$f_l\left( x \right)$，并提取channel-wise的means \(\mu _{l,c}\):

To extract the data distribution \(E_{l}^{t}\) and reduce the calculation and memory overhead of the extraction process, we use representative statistics to represent complex data distribution. Existing methods usually obtain statistical information by extracting higher-order moments of samples \cite{HoMM: Higherorder Moment Matching for Unsupervised Domain Adaptation, Central Moment Discrepancy (CMD) for Domain-Invariant Representation Learning.}. However, the input data batch size may be small in mobile, making it difficult to extract accurate data distribution from higher-order moments. We separately process the \(l\)th layer output $f_l\left( x \right)$ and extract channel-wise means \(\mu _{l,c}\) and variances \(\sigma _{l,c}^{2}\), as Eq.~\ref{m1-2} and Eq.~\ref{m1-3},
\begin{equation} \label{m1-2}
    \mu _c\left( f_l\left( x \right) \right) =\frac{1}{N}\sum_{i=1}^N{f_{l,c}^{i}\left( x \right)},
\end{equation}
\begin{equation} \label{m1-3}
\sigma _{c}^{2}\left( f_l\left( x \right) \right) =\frac{1}{N}\sum_{i=1}^N{\left( f_{l,c}^{i}\left( x \right) -\mu _c\left( f_l\left( x \right) \right) \right) ^2}.
\end{equation}
%通过计算每个通道的\(\mu _{l,c}\)和\(\sigma _{l,c}^{2}\)并将它们连接，我们得到第\(l\)层输出对于输入分布$C_t$的分布表征\(E_{l}^{t}\)：
By calculating the \(\mu _{l,c}\) and \(\sigma _{l,c}^{2}\) for each channel and concatenating them, we extract the distribution representation \(E_{l}^{t}\) of the \(l\)th layer output with respect to the input distribution $C_t$, as Eq.~\ref{m1-4},
\begin{equation} \label{m1-4}
E_{l}^{t}=\left[ \mu _1\left( f_l\left( x \right) \right) ,\ \sigma _{1}^{2}\left( f_l\left( x \right) \right) ,\ .\ .\ .\ ,\ \mu _c\left( f_l\left( x \right) \right) ,\,\,\sigma _{1}^{2}\left( f_l\left( x \right) \right) \right].
\end{equation}
%如图xx所示，以图像数据为例，这种分布表征能够有效表示当前图像的风格与语义信息。由于模型需要不断适应新的场景，因此代表模型已经适应的历史分布$H$也需要随着模型的适应而逐渐更新。在连续场景的适应中，我们利用an exponential moving average technique来逐渐更新历史分布表征：
As shown in Fig. xx, the distribution embedding can effectively represent the style and semantic information of the current input. Since the model needs to continuously adapt to new scenes, the historical distribution embedding \(E_{l}^{H}\) that the model has already adapted also needs to be gradually updated. In adaptation of continuous scenes, we use an exponential moving average technique~\cite{} to update the historical distribution embedding \(E_{l}^{H}\), as Eq.~\ref{m1-5},
\begin{equation} \label{m1-5}
E_{l}^{t}=\alpha E_{l}^{t-1}+\left( 1-\alpha \right) E_{l}^{H}.
\end{equation}
%为了在缺少数据标签的情况下训练模型，现有的测试时适应方法通常以模型最后一层输出的熵作为损失函数来优化模型。但这种方法忽略了数据本身包含的分布信息和其它层的输出信息，难以充分利用小批次数据的有限信息。为了对齐新旧场景数据下模型输出的分布差异，我们以减小模型每层的当前输出分布$E_{i}^{t}$和历史输出$E_{i}^{H}$之间的KL-divergence为优化目标，并累加所有层的KL-divergence作为损失函数：
To complete model adaptation without labels, existing test-time adaptation methods usually use the entropy of the model's last layer output as the loss function to optimize the model. However, this method ignores the distribution information contained in data and the output information of other layers, making it difficult to fully utilize the limited knowledge of small batch data. To align the distribution differences of layer outputs between current and historical scene data, we aim to minimize the KL-divergence between the current output embedding $E_{i}^{t}$ and historical output embedding $E_{i}^{H}$ of each layer, and sum the KL-divergence of all layers as the loss function, as Eq.~\ref{m1-6},
\begin{equation} \label{m1-6}
L=\sum_{i=1}^I{D_{KL}\left( E_{i}^{H}\lVert E_{i}^{t} \right.)}.
\end{equation}
%由于逐个通道而非逐个参数提取一阶统计量和二阶统计量，并且重用了forward的计算结果，我们提出的层精度重要性评估方法是计算友好和内存友好的。对于vgg16，resnet50和mobilenetv2而言，评估batchsize为16的数据的层精度重要性的计算开销分别约为推理的xx%，xx%和xx%。储存在设备中的历史数据的分布表征与层数和通道数相关。对于resnet50而言，$H$的大小通常在xxKB左右。此外，如果将分布提取过程和forward并行计算能够进一步减小评估带来的额外开销。
By extracting the first-order and second-order statistics channel-wise rather than parameter-wise and reusing the forward intermediate results, our proposed accuracy importance profiler is computationally and memory friendly. For VGG16, ResNet50, and MobileNetV2, the evaluating computation overhead with a batch size of 16 is approximately xx\%, xx\%, and xx\% of the inference, respectively. The historical data distribution representation stored in the device is related to the number of layers and channels. For ResNet50, the size of $H$ is usually around xxKB. Moreover, if the distribution extraction process and forward computation are performed in parallel, the additional overhead of evaluation can be further reduced.


\subsection{Latency-Overhead Profiler (LOP)}
% 为了准确的评估各层更新所需要的时延，我们同样构建了一个基于实时硬件信息的在线Profiler。
To accurately evaluate the latency required for updating each layer, we also build an online profiler based on runtime hardware information.
%每层的实际运行时延在不同的硬件条件下会发生改变\cite{}。测试时适应通常在设备并行执行其他任务时进行，此时分配给每个应用程序的硬件资源是高度动态的。这意味着适应进程需要和忙碌设备上更多的其他进程同时竞争设备资源，这给每层的实际执行时延带来了更多的不确定性。
The execution latency of each layer may vary under different hardware conditions \cite{}. Test-time adaptation is usually carried out when the device is performing other tasks in parallel and the hardware resources allocated to each application are highly dynamic. Therefore, the adaptation process needs to compete for device resources with more other processes which brings more uncertainty to the actual execution latency of each layer.
%为了准确评估动态硬件条件下的层时延，需要首先分析影响层时延的各个组成部分的硬件条件因素。在深度模型的推理和训练过程中，每一层在设备理想环境下的总时延主要由计算时延和访存时延组成：
To evaluate the layer latency under dynamic hardware conditions, we first analyze the factors that affect different components of layer latency. The total latency of layer $l$ under offline device condition is mainly composed of computation latency $T_{F}^{l}$ and memory access latency $T_{M}^{l}$:
$$
T_{off}^{l}=T_{F}^{l}+T_{M}^{l}
$$ 
%然而当设备实际运行时，每一层的计算时延和访存时延受当前的主频和cache-hit-rate等不同因素影响而变化。因此第\(l\)层的在线运行时延T_{on}^{l}在运行环境下与理想环境下的离线时延T_{off}^{l}关系可建模为：\(T_{on}^{l}=\pi _1\cdot T_{F}^{l}+\pi _2\cdot T_{M}^{l}\)。其中\(pi_1\)，\(pi_1\)分别为计算时延和访存时延在实际运行条件下的相比于理想环境下的时延的增加倍数，我们称之为计算膨胀系数和访存膨胀系数。
However, when the device is running, $T_{F}^{l}$ and $T_{M}^{l}$ are affected by different factors such as the current CPU/GPU usage and cache-hit-rate. Therefore, the online latency $T_{on}^{l}$ of the \(l\)th layer in running device condition can be modeled in relation to the offline latency $T_{off}^{l}$ in ideal device condition: \(T_{on}^{l}=\pi _1\cdot T_{F}^{l}+\pi _2\cdot T_{M}^{l}\). Here, \(pi_1\) and \(pi_2\) are the increased multiples of $T_{F}^{l}$ and $T_{M}^{l}$, which we call the computation inflation factor and memory access inflation factor, respectively.
$$
T_{on}^{l}=\pi _1\cdot T_{F}^{l}+\pi _2\cdot T_{M}^{l}
$$

%每层的计算时延主要受该层的浮点运算次数和设备单位时间内能够执行浮点运算次数的影响。对于相同层和相同设备而言，影响单位时间内能够执行该层的浮点运算次数的因素主要包含竞争进程数和硬件温度（例如CPU、GPU）。%\textbf{竞争进程数}：资源受限的移动设备通常依赖CPU或GPU完成计算。以CPU为例，设备操作系统内核（如Linux）默认采用Round Robin scheduling（RR）公平调度计算进程。导致当竞争进程数上升时，当前计算进程的等待时间也会随之上升。%\textbf{硬件温度}：当设备CPU温度升高时，动态电压频率缩放（DVFS）会通过降低主频控制功耗。这会导致当前计算进程的计算时间上升。

The computation latency $T_{F}^{l}$ of layer $l$ is mainly affected by the number of the Multiply–Accumulate(MACs) the device can perform for layer $l$ per second. For the same layer and device, the factors that affect the number of MACs that can be performed per second include the number of competing processes and hardware temperature.
\textbf{Competing process number}: Resource-limited mobile devices usually rely on CPUs or GPUs for computation. Taking the CPU as an example, the device operating system kernel (such as Linux) adopts Round Robin scheduling (RR) by default to fairly schedule computing processes. As a result, when the number of competing processes increases, the waiting time of the adaptation computing process also increases.
\textbf{Hardware temperature}: When the device's CPU/GPU temperature rises, dynamic voltage frequency scaling (DVFS) controls power consumption by lowering the clock frequency. This leads to an increase in the computation time of the adaptation computing process.

%因此，竞争进程数为\(n\)，CPU或GPU温度为\(tem_on\)时，计算膨胀系数\(pi_1\)为：
Therefore, when the number of competing processes is \(n\) and the CPU or GPU temperature is \(tem_on\), the computation inflation factor \(pi_1\) is:
$$
\pi _1=\frac{freq\left( tem_{off} \right)}{freq\left( tem_{on} \right)}\cdot \left[ 1+f\left( n \right) \right] 
$$
%其中\(f\left( n \right)\)是关于竞争进程数的线性函数，受轮循时间大小和切换进程开销决定。\(freq\)是特定设备CPU频率关于温度的降频函数。 \(f\left( n \right)\)函数可在训练前离线快速测量并拟合， \(freq\)函数可通过CPU或GPU的DVFS策略感知。
where \(f\left( n \right)\) is a linear function related to the number of competing processes \(n\), determined by the overhead of switching processes. \(freq\) is a down-frequency function of the specific device's CPU/GPU frequency with respect to temperature. The \(f\left( n \right)\) function can be quickly measured and fitted offline before deployment by simulating competing processes, while the \(freq\) function can be perceived through the CPU/GPU DVFS strategy.

%每层的访存时延主要受该层的访存量和访存带宽的影响。访存时延主要受缓存命中率影响。访问数据时，如果在缓存中未命中数据，那么需要退回到内存中访问数据并基于远低于缓存带宽的内存带宽传输数据到计算单元。设备运行时多个进程可能互相占用缓存区域从而降低适应进程的缓存命中率，增加内存访问时延。基于设备的缓存带宽\(b_cache\)和内存DRAM带宽\(b_dram\)，访存膨胀系数\(pi_2\)为：
The memory access latency $T_{M}^{l}$ is mainly affected by the cache-hit-rate $\varphi$. 
If target data is not found in cache, process needs to go back to DRAM to access and transfer it to the computing unit based on DRAM bandwidth, which is much lower than cache bandwidth. When the device is running, multiple processes may share the cache area, reducing the cache-hit-rate of the adaptation process and increasing the memory access latency.
Based on device cache bandwidth \(b_cache\) and DRAM bandwidth \(b_dram\), the memory access inflation factor \(pi_2\) is:
$$
\pi _2=\frac{\left[ \varphi \cdot b_{cache}+\left( 1-\varphi \right) \cdot b_{dram} \right]}{b_{cache}}
$$
%因此，第\(l\)层的运行时延和离线时延关系为：
Therefore, the relationship between the runtime latency $T_{on}^{l}$ and offline latency $T_{off}^{l}$ of the \(l\)th layer is:
$$
T_{on}^{l}=\frac{\pi _1\cdot \eta _l+\pi _2}{\eta _l+1}\cdot T_{off}^{l}
$$
$$
\eta _l=\frac{T_{F}^{l}}{T_{M}^{l}}=\frac{F^l}{\delta _M}\cdot \frac{\delta _F}{M^l}
$$

%其中，\(N^l\) 和\(M^l\) 分别为第\(l\)层的浮点运算次数和访存量， $\delta _M$和$\delta _F$分别为单位访存时间和单次浮点运算时间。
where \(F^l\) and \(M^l\) are the number of MACs and memory access amount of the \(l\)th layer, respectively. $\delta _M$ and $\delta _F$ represent the unit memory access time and unit MAC time, respectively.


\begin{align*}\label{1}
  & T_{on}^{l}=\pi _1\cdot T_{F}^{l}+\pi _2\cdot T_{M}^{l} \\
  & =\left( \frac{\eta _l}{\eta _l+1}\cdot \pi _1+\frac{1}{\eta _l+1}\cdot \pi _2 \right) \cdot T_{off}^{l} \\
\end{align*}

%在公式9中，不同层在时延预测时，设备条件$pi _1$和$pi _2$保持相同，单位计算和访存时间$\delta _M$,$\delta _F$也相同，唯一不同的是$\frac{F^l}{M^l}$。实际上，$\frac{F^l}{M^l}$表示层的计算密度\cite{williams2008auto}，即每层的浮点运算次数与访存量之比。不同的层具有不同的计算密度，如图xx所示，卷积层和线性层的计算密度较高，而激活层和池化层的计算密度较低。从公式9中可以看出，计算密度越高的层，其运行时延受到计算膨胀系数$pi _1$的影响越大；计算密度越低的层，其运行时延受到访存膨胀系数$pi _2$的影响越大。如图xx所示，不同硬件条件下，各层时延的大小关系甚至可能出现逆转。因此，在线执行时延能更准确地反映每层实际执行时延的大小次序，从而实现精确的稀疏更新策略搜索。需要指出的是，尽管激活层等non-parameter层不参与更新，但仍需参与反向传播以计算梯度，因此也需要对这些层进行在线时延预测。

%在实际部署SwiftTTA时，首先需要在设备空闲时测量静态层的时延。在设备运行过程中，根据当前硬件条件计算膨胀系数$pi _1$和$pi _2$，进而得到当前设备状态下每层的在线运执行时延。通过对在线时延进行动态建模，我们可以在硬件条件实时发生变化时，预测不同层由于计算密度不同而产生的不同程度的时延变化。这为稀疏更新搜索算法提供了准确的层时延信息，从而使实际适应时延符合预期的加速效果。
As the computation inflation factor $pi _1$ and memory access inflation factor $pi _2$ independently affect the computation latency $T_{F}^{l}$ and memory access latency $T_{M}^{l}$, runtime latencys' change scale for layers with different arithmetic intensity\cite{williams2008auto} is not the same when hardware conditions dynamically change. 
\frac{F^l}{M^l} is the 
The computation density is an important metric of a layer, which is the ratio of floating-point operations to memory access volume, i.e., xx/xx (write the formula). Formula 9 shows that the higher the computation density of a layer (such as a convolutional layer), the greater the impact of the computation inflation factor on the runtime latency; the lower the computation density of a layer (such as an activation layer), the greater the impact of the access inflation factor on the runtime latency. In addition, the computation density of layers of the same type may also differ, as shown in the figure. It should be noted that although activation layers do not have weights and do not participate in weight updates, they still need to participate in the calculation of gradients during backpropagation, and therefore need to be considered within the range of layer latency.



==> body/others/related_work.tex <==

\textbf{Test-time adaptation}.
\TODO{stop here}
%这些研究通过修改原网络并添加新网络结构，降低持续学习在移动端的内存资源占用。
%TinyTL\cite{} 在冻结原网络权重W的同时添加memory-efficient bias module与原网络模块并联，减小了中间激活大小，从而大幅降低了网络训练内存占用。但bias module的添加会额外增加计算量，从而增加训练时延和能耗。
%这类设计并没有考虑到迁移学习的时延，并且更新整个模型会导致在新场景上的过拟合和泛化能力降低的问题。并会随着多次迁移从而导致精度快速下降甚至崩塌。


\textbf{On-device training}. 
%足够的内存是决定训练是否成功的关键因素。因此现有的on-device training技术主要针对终端设备紧张的内存资源设计训练优化方法。 Lin等人\cite{lin2022device}通过设计quantization-aware scaling、sparse update算法和tiny training engine将图像分类的训练内存压缩到了256KB以下。Wang等人\cite{wang2022melon}基于MNN\cite{}框架和内存池设计将重计算和micro-batch技术应用于手机设备, 大幅降低了训练内存。随后，Gim等人\cite{gim2022memory}结合operator and graph-level optimizations和重计算等技术在手机上实现了memory-efficient DNN training.最近，Xu等人提出了DSP-offloading based mixed-precision，通过量化技术优化训练内存和时延。而如图xxx所示，量化能够降低时延并节省内存，但也会大幅降低多轮迁移学习后的精度。而其他on-device training研究则只考虑了内存优化而没有优化时延，甚至会因为重计算和micro-batch技术而大幅增加训练时延。此外Meva作为一种训练模式的优化，和量化、micro-batch、operator and graph-level optimizations等大部分优化技术并不冲突。在任务对时延或内存有极端需求时可以与这些技术耦合使用以进一步提升性能。
A sufficient amount of memory is a key factor in determining the success of training. Therefore, existing on-device training techniques mainly focus on designing training optimization methods for terminal devices with limited memory resources. For example, Lin et al. \cite{lin2022device} compressed the training memory for image classification to less than 256KB by designing quantization-aware scaling, sparse update algorithms, and a tiny training engine. Wang et al. \cite{wang2022melon} applied recomputation and micro-batch techniques to mobile devices based on the MNN framework and memory pool design, significantly reducing training memory. Subsequently, Gim et al. \cite{gim2022memory} combined operator and graph-level optimizations and recomputation techniques to achieve memory-efficient DNN training on mobile devices. Recently, Xu et al. proposed a mixed-precision method based on DSP offloading, which optimizes training memory and latency through quantization techniques. As shown in Figure \ref{}, quantization techniques can reduce latency and save memory, but they can also significantly reduce accuracy after multiple rounds of transfer learning. On the other hand, other on-device training research only considers memory optimization without optimizing latency, and may even significantly increase training latency due to recomputation and micro-batch techniques. In addition, Meva, as an optimization of the training mode, does not conflict with most optimization techniques such as quantization, micro-batch, operator, and graph-level optimizations. When there is an extreme demand for latency or memory in a task, these techniques can be combined with Meva to further enhance performance.


\textbf{Partial updating}
\TODO{optimize}
%为了应对移动端的数据变化，模型需要高效演化（即迁移学习）以学习新场景。根据update网络的不同部分，演化方法可分为三类。（i）\textit{Fixed updating} 是最简单的演化技术，模型演化时只训练最后一层或BN层。但演化精度较差，并且难以应对多种数据shift。\textit{Accuracy-aware updating}分别对网络每一层进行单独更新，计算对应精度提升，并通过搜索算法选择精度提升之和最高的层组合进行更新。然而，多次更新和搜索过程具有很高的时延和能耗成本（几倍于原本的训练），因此只能在部署前离线计算更新方案。因此，固定执行updating方案也无法应对多种数据shift。\textit{Shift-aware updating}根据数据发生的shift类型微调模型的特定部分。但这种方法需要显式提供当前数据shift类别而无法自动检测。相比这些方法，MevaTrain能够通过提取图像和历史场景之间的feature diversity判断当前数据的shift kind并判断需要更新的网络模块。需要注意的是，这些过程都是实时的，几乎不会带来额外计算时延和能耗。
To cope with data shift, the model needs to evolve efficiently to learn new mobile scenarios, i.e., transfer learning). According to different updating part of the model, evolution methods can be divided into three categories. (i) \textit{Fixed updating} is the simplest evolution technique, where only the last layer\cite{} or BN layer\cite{} is updated during evolution. However, the evolution accuracy is poor, and it is difficult to deal with different data shifts. (ii) \textit{Accuracy-aware updating} updates each layer of the network separately, calculates the corresponding accuracy improvement, and selects the layer combination with the highest sum of accuracy improvements for updating through a search algorithm. However, the multiple updating and search processes bring high latency and energy consumption (several times that of the original training\cite{}), so the update plan can only be computed offline before deployment. And fixed updating plans also cannot cope with multiple data shifts. (iii) \textit{Shift-aware updating} fine-tunes specific parts of the model based on the type of occurs data shift. However, it requires explicit provision of the current data shift category and cannot detect it automatically. MevaTrain can detect the shift kind of current data and determine the network block that need to be updated by extracting feature diversity between current images and historical scenes. It should be noted that these processes are real-time and almost do not bring extra computational latency and energy consumption.



%第一类：只微调模型最后一层或者BN层等。无法抗遗忘；无法应对多类型场景。对于多个shift kinds，精度不足，需要小实验
%第二类：Shift-aware finetuning：需要提供当前数据的shift kind信息，无法实现自适应检测。必须是given shift kind，我们是实时检测shift kind
%第三类：Accuracy-aware finetuning：确定最佳SU方案需要大量额外计算和搜索成本，应用在移动端会大幅提高任务时延和能耗；这一种是offline，速度不行。我们是online。
%OURs：shift-aware runtime directional updating：我们是runtime shift检测类型，根据移动端当前数据流实时检测出shift kind（用常用词）；





















